NGC 5128 globular cluster candidates out to 150 kpc: a comprehensive catalog from Gaia and ground based data

We present a new catalog of 40502 globular cluster (GC) candidates in NGC 5128 out to a projected radius of $\sim$150 kpc, based on data from the Panoramic Imaging Survey of Centaurus and Sculptor (PISCeS), Gaia Data Release 2, and the NOAO Source Catalog. Ranking these candidates based on the likelihood that they are true GCs, we find that approximately 1900 belong to our top two ranking categories and should be the highest priority for spectroscopic follow-up for confirmation. Taking into account our new data and a vetting of previous GC catalogs, we estimate a total GC population of $1450 \pm 160$ GCs. We show that a substantial number of sources previously argued to be low-velocity GCs are instead foreground stars, reducing the inferred GC velocity dispersion. This work showcases the power of Gaia to identify slightly extended sources at the $\sim 4$ Mpc distance of NGC 5128, enabling accurate identification of GCs throughout the entire extended halo, not just the inner regions that have been the focus of most previous work.

==> table_all.tex <==
\begin{sidewaystable}
\tiny
\centering
\caption{PISCeS sources around NGC~5128}
\renewcommand{\tabcolsep}{1.05mm}
  
\begin{tabular}{c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c}
\hline \hline
ID & Discovery & PISCeS R.A. & PISCeS Decl.   &  PISCeS g  & PISCeS r  &  $C_{3-6, g}$ & $C_{3-6, r} $ & better &  structure  &  Gaia R.A. & Gaia Decl. & Gaia G & $\mu_{\alpha*}$ &  $\mu_{\delta}$  & $\varpi$ &  AEN   &  BR$_{\rm exc.}$ &  NSC $u$ & NSC $g$ & NSC $r$  & NSC $i$ & NSC $z$  &  NSC $u_{err}$ & NSC $g_{err}$ & NSC $r_{err}$  & NSC $i_{err}$ & NSC $z_{err}$  &  $(u-r)_0$  & $(r-z)_0$ &$\mu$  & $\varpi$  &  AEN  &  BPRP  & Color & Total &  data  &  confirmed &  references  \\
(H20) &  ID*  & (J2000) & (J2000) & (mag) & (mag) &   &   & seeing  & $\mathscr{L}$ & (J2000) & (J2000) & (mag) &  (mas/yr) &  (mas/yr) & (mas) & (mas)  &    & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) &  (mag) & (mag) & $\mathscr{L}$ & $\mathscr{L}$  & $\mathscr{L}$  & $\mathscr{L}$  & $\mathscr{L}$  & $\mathscr{L}$  & category &     &       \\
\hline
H20-1 &  -  & 200.765133 & -42.862403 & 21.61$\pm$0.02 & 20.16$\pm$0.01 & -0.5 & -0.4 & r & 1.0 & 200.76507 & -42.862429 & -5.02$\pm$1.88 & 4.01$\pm$1.47 & 0.69$\pm$0.99 & 3.82 & 1.49 & 0.000 & 21.40 & 20.06 & 19.48 & 19.21 & 0.000 & 0.003 & 0.001 & 0.001 & 0.019 & 0.00 & 0.00 & 0.00 & 0.48 & 0.99 & 0.56 &  - & 0.00 &  - & -  &  -  \\
H20-2 &  -  & 200.699970 & -43.058100 & 20.75$\pm$0.01 & 20.02$\pm$0.01 & 1.50 & 0.32 & r & 1.0 & 200.69993 & -43.058129 & -3.86$\pm$1.37 & 0.77$\pm$1.68 & 0.13$\pm$0.76 & 0.0 & 1.30 & 21.94 & 20.53 & 20.09 & 19.91 & 19.86 & 0.022 & 0.002 & 0.001 & 0.002 & 0.012 & 1.54 & 0.08 & 0.01 & 0.85 & 0.02 & 0.20 & 0.02 & 0.00 &  - & -  &  -  \\
H20-3 &  -  & 200.758579 & -42.925393 & 20.23$\pm$0.01 & 19.67$\pm$0.01 & 0.54 & 0.13 & r & 1.0 & 200.75854 & -42.925424 & -2.66$\pm$0.90 & -0.67$\pm$0.72 & 0.36$\pm$0.48 & 0.34 & 1.30 & 21.48 & 20.14 & 19.68 & 19.43 & 19.38 & 0.016 & 0.002 & 0.001 & 0.001 & 0.011 & 1.52 & 0.15 & 0.00 & 0.45 & 0.05 & 0.25 & 0.02 & 0.00 &  - & -  &  -  \\
H20-4 &  -  & 200.958785 & -43.030524 & 20.32$\pm$0.01 & 18.88$\pm$0.01 & -1.3 & -1.7 & r & 1.0 & 200.95872 & -43.030562 & -10.36$\pm$0.38 & -6.36$\pm$0.35 & 1.93$\pm$0.34 & 0.35 & 1.48 & 22.94 & 20.09 & 18.73 & 17.42 & 16.86 & 0.069 & 0.001 & 0.000 & 0.000 & 0.003 & 3.95 & 1.73 & 0.00 & 0.00 & 0.34 & 0.99 & 0.02 & 0.00 &  - & -  &  -  \\
H20-5 &  -  & 200.609066 & -43.090697 & 19.67$\pm$0.01 & 18.81$\pm$0.01 & 0.77 & 0.79 & r & 1.0 & 200.60904 & -43.090715 & -4.69$\pm$0.59 & 1.72$\pm$0.44 & 1.07$\pm$0.27 & 0.0 & 1.30 & 21.51 & 19.52 & 18.83 & 18.57 & 18.46 & 0.016 & 0.001 & 0.000 & 0.000 & 0.004 & 2.38 & 0.20 & 0.00 & 0.00 & 0.02 & 0.47 & 0.02 & 0.00 &  - & -  &  -  \\
H20-6 &  -  & 200.766650 & -42.844439 & 19.78$\pm$0.01 & 18.45$\pm$0.01 & -2.7 & -0.6 & r & 1.0 & 200.76659 & -42.844482 & -4.15$\pm$0.49 & -10.99$\pm$0.31 & 0.19$\pm$0.20 & 0.16 & 1.33 & 22.31 & 19.59 & 18.38 & 17.86 & 17.63 & 0.038 & 0.001 & 0.000 & 0.000 & 0.003 & 3.66 & 0.60 & 0.00 & 0.33 & 0.07 & 0.84 & 0.02 & 0.00 &  - & -  &  -  \\
H20-7 &  -  & 200.818849 & -43.106020 & 19.19$\pm$0.01 & 18.59$\pm$0.01 & -0.5 & -0.9 & r & 1.0 & 200.81881 & -43.106053 & -6.07$\pm$0.45 & 1.15$\pm$0.34 & 0.14$\pm$0.26 & 0.0 & 1.28 & 20.55 & 19.09 & 18.60 & 18.39 & 18.32 & 0.009 & 0.001 & 0.000 & 0.000 & 0.004 & 1.66 & 0.14 & 0.00 & 0.58 & 0.02 & 0.46 & 0.02 & 0.00 &  - & -  &  -  \\
H20-8 &  -  & 200.658255 & -42.959613 & 21.79$\pm$0.02 & 20.71$\pm$0.02 & 6.29 & 7.80 & r & 0.0 &  - & - & - & - & - & - & - & - &  0.000 & 21.68 & 20.44 & 20.01 & 19.82 & 0.000 & 0.005 & 0.001 & 0.001 & 0.019 & 0.00 & 0.00 &  - & - & - & - &  - & 0.00 &  - & -  &  -  \\
H20-9 &  -  & 200.731413 & -43.107674 & 21.61$\pm$0.02 & 20.59$\pm$0.02 & -1.0 & 0.31 & r & 1.0 & 200.73136 & -43.107704 & -12.38$\pm$2.04 & 1.38$\pm$2.03 & 1.05$\pm$1.22 & 0.0 & 1.95 & 0.000 & 21.47 & 20.56 & 20.15 & 19.96 & 0.000 & 0.004 & 0.002 & 0.002 & 0.017 & 0.00 & 0.00 & 0.00 & 0.39 & 0.02 & 0.83 &  - & 0.00 &  - & -  &  -  \\
H20-10 &  -  & 200.785866 & -42.960638 & 21.87$\pm$0.03 & 20.25$\pm$0.01 & -2.1 & -1.6 & r & 1.0 & 200.78579 & -42.960671 & -8.40$\pm$0.82 & -0.33$\pm$0.73 & 1.79$\pm$0.45 & 1.10 & 1.65 & 0.000 & 21.63 & 20.07 & 18.61 & 17.96 & 0.000 & 0.003 & 0.001 & 0.000 & 0.003 & 0.00 & 0.00 & 0.00 & 0.00 & 0.56 & 0.98 &  - & 0.00 &  - & -  &  -  \\
H20-11 &  -  & 200.738238 & -43.057925 & 21.13$\pm$0.01 & 20.24$\pm$0.01 & -0.4 & -0.4 & r & 1.0 & 200.73818 & -43.057955 & -11.43$\pm$1.88 & 1.23$\pm$3.09 & -0.52$\pm$1.24 & 0.0 & 1.50 & 23.25 & 21.02 & 20.20 & 19.88 & 19.71 & 0.081 & 0.003 & 0.001 & 0.002 & 0.013 & 2.75 & 0.34 & 0.00 & 0.67 & 0.02 & 0.50 & 0.02 & 0.00 &  - & -  &  -  \\
H20-12 &  -  & 200.615473 & -42.888031 & 18.97$\pm$0.01 & 18.48$\pm$0.01 & 1.54 & 1.83 & r & 1.0 & 200.61545 & -42.888066 & 0.75$\pm$0.43 & -10.71$\pm$0.34 & -0.12$\pm$0.22 & 0.0 & 1.27 & 20.07 & 18.87 & 18.48 & 18.31 & 18.29 & 0.006 & 0.001 & 0.000 & 0.000 & 0.004 & 1.32 & 0.05 & 0.00 & 0.59 & 0.02 & 0.37 & 0.02 & 0.00 &  - & -  &  -  \\
H20-13 &          245$^i$ & 201.042738 & -42.962687 & 21.68$\pm$0.02 & 20.99$\pm$0.03 & 17.41 & 21.40 & r & 0.0 &  - & - & - & - & - & - & - & - &  0.000 & 21.41 & 20.74 & 20.47 & 20.40 & 0.000 & 0.004 & 0.003 & 0.003 & 0.034 & 0.00 & 0.00 &  - & - & - & - &  - & 0.00 &  - & -  &  i  \\
H20-14 &  -  & 200.975085 & -43.069110 & 21.86$\pm$0.03 & 20.53$\pm$0.02 & -1.5 & -0.5 & r & 1.0 & 200.97503 & -43.069137 &  - &  - &  - & 3.87 & 1.62 & 0.000 & 21.73 & 20.48 & 19.95 & 19.70 & 0.000 & 0.005 & 0.001 & 0.002 & 0.011 & 0.00 & 0.00 &  - &  - & 0.95 & 0.56 &  - & 0.00 &  - & -  &  -  \\
H20-15 &  -  & 201.035500 & -42.927712 & 21.09$\pm$0.01 & 19.56$\pm$0.01 & -0.7 & 0.35 & r & 1.0 & 201.03543 & -42.927743 & -8.66$\pm$0.52 & -7.08$\pm$0.46 & 2.58$\pm$0.32 & 0.81 & 1.64 & 23.22 & 20.82 & 19.38 & 17.86 & 17.20 & 0.104 & 0.002 & 0.000 & 0.000 & 0.002 & 3.58 & 2.04 & 0.00 & 0.00 & 0.73 & 0.99 & 0.02 & 0.00 &  - & -  &  -  \\
H20-16 &  -  & 200.849185 & -43.105918 & 19.51$\pm$0.01 & 18.69$\pm$0.01 & -1.0 & -0.6 & r & 1.0 & 200.84914 & -43.105966 & -4.82$\pm$0.46 & -10.82$\pm$0.37 & 0.30$\pm$0.28 & 0.17 & 1.34 & 21.45 & 19.37 & 18.70 & 18.42 & 18.31 & 0.018 & 0.001 & 0.000 & 0.000 & 0.004 & 2.47 & 0.24 & 0.00 & 0.29 & 0.05 & 0.69 & 0.02 & 0.00 &  - & -  &  -  \\
H20-17 &  -  & 200.732613 & -42.825415 & 21.76$\pm$0.02 & 20.31$\pm$0.01 & -1.5 & -0.6 & g & 1.0 & 200.73254 & -42.825444 & -3.94$\pm$1.76 & 0.90$\pm$0.91 & -0.01$\pm$0.64 & 0.0 & 1.60 & 0.000 & 21.55 & 20.18 & 19.36 & 19.01 & 0.000 & 0.003 & 0.001 & 0.001 & 0.008 & 0.00 & 0.00 & 0.06 & 0.98 & 0.02 & 0.77 &  - & 0.00 &  - & -  &  -  \\
H20-18 &  -  & 200.925840 & -43.026421 & 19.18$\pm$0.01 & 18.24$\pm$0.01 & -1.7 & 0.49 & r & 1.0 & 200.92579 & -43.026455 & -9.61$\pm$0.44 & -0.94$\pm$0.35 & 0.50$\pm$0.28 & 0.67 & 1.25 & 21.49 & 19.02 & 18.17 & 17.89 & 17.78 & 0.023 & 0.001 & 0.000 & 0.000 & 0.005 & 3.06 & 0.26 & 0.00 & 0.07 & 0.89 & 0.35 & 0.02 & 0.00 &  - & -  &  -  \\
H20-19 &  -  & 200.662211 & -42.990680 & 20.61$\pm$0.01 & 20.14$\pm$0.01 & -0.7 & -0.3 & r & 1.0 & 200.66217 & -42.990714 & -6.51$\pm$1.34 & -2.52$\pm$1.43 & 0.30$\pm$0.86 & 0.82 & 1.24 & 21.81 & 20.54 & 20.14 & 19.98 & 19.94 & 0.021 & 0.001 & 0.001 & 0.001 & 0.016 & 1.39 & 0.05 & 0.00 & 0.72 & 0.15 & 0.11 & 0.02 & 0.00 &  - & -  &  -  \\
H20-20 &  -  & 200.627079 & -42.923904 & 21.90$\pm$0.02 & 21.27$\pm$0.04 & -0.2 & 0.04 & r & 1.0 &  - & - & - & - & - & - & - & - &  23.40 & 21.79 & 21.31 & 21.15 & 21.25 & 0.113 & 0.004 & 0.003 & 0.004 & 0.042 & 1.82 & -0.0 &  - & - & - & - & 0.02 & 0.00 &  - & -  &  -  \\
H20-21 &  -  & 200.974466 & -43.143795 & 20.38$\pm$0.01 & 19.73$\pm$0.01 & -0.5 & -0.5 & r & 1.0 & 200.97441 & -43.143831 & -5.33$\pm$1.05 & 0.47$\pm$0.80 & 0.58$\pm$0.70 & 0.0 & 1.25 & 21.95 & 20.30 & 19.73 & 19.51 & 19.44 & 0.023 & 0.001 & 0.001 & 0.001 & 0.009 & 1.96 & 0.15 & 0.00 & 0.41 & 0.02 & 0.16 & 0.02 & 0.00 &  - & -  &  -  \\
H20-22 &  -  & 200.852073 & -42.889980 & 21.30$\pm$0.01 & 20.44$\pm$0.01 & -0.7 & -0.5 & r & 1.0 & 200.85203 & -42.890007 &  - &  - &  - & 0.0 & 1.79 & 23.29 & 21.17 & 20.43 & 20.16 & 20.05 & 0.089 & 0.002 & 0.001 & 0.002 & 0.018 & 2.58 & 0.22 &  - &  - & 0.02 & 0.79 & 0.02 & 0.00 &  - & -  &  -  \\
H20-23 &  -  & 200.726924 & -42.923940 & 19.25$\pm$0.01 & 18.66$\pm$0.01 & -0.3 & -0.9 & r & 1.0 & 200.72687 & -42.923975 & -12.04$\pm$0.57 & -2.86$\pm$0.41 & 0.48$\pm$0.27 & 0.0 & 1.30 & 20.61 & 19.13 & 18.68 & 18.49 & 18.47 & 0.011 & 0.001 & 0.000 & 0.000 & 0.006 & 1.65 & 0.07 & 0.00 & 0.07 & 0.02 & 0.51 & 0.02 & 0.00 &  - & -  &  -  \\
H20-24 &  -  & 200.799199 & -42.824878 & 21.97$\pm$0.03 & 20.66$\pm$0.02 & 19.23 & 23.48 & r & 0.0 &  - & - & - & - & - & - & - & - &  0.000 & 21.39 & 20.05 & 19.43 & 19.12 & 0.000 & 0.006 & 0.002 & 0.002 & 0.015 & 0.00 & 0.00 &  - & - & - & - &  - & 0.00 &  - & -  &  -  \\
H20-25 &  -  & 200.865180 & -43.026323 & 21.72$\pm$0.02 & 20.65$\pm$0.02 & -1.7 & -1.8 & r & 1.0 & 200.86513 & -43.026363 & -4.85$\pm$2.66 & -3.20$\pm$2.91 & -0.76$\pm$1.30 & 3.43 & 1.64 & 0.000 & 21.57 & 20.62 & 20.26 & 20.14 & 0.000 & 0.003 & 0.002 & 0.002 & 0.032 & 0.00 & 0.00 & 0.10 & 0.55 & 0.74 & 0.48 &  - & 0.00 &  - & -  &  -  \\
H20-26 &  -  & 200.901734 & -43.026201 & 19.10$\pm$0.01 & 18.16$\pm$0.01 & 1.64 & 1.56 & r & 1.0 & 200.90166 & -43.026231 & -12.08$\pm$0.90 & 4.11$\pm$0.73 & 3.78$\pm$0.59 & 2.20 & 1.48 & 21.02 & 18.96 & 18.15 & 17.84 & 17.70 & 0.014 & 0.001 & 0.000 & 0.000 & 0.005 & 2.60 & 0.31 & 0.00 & 0.00 & 1.00 & 0.99 & 0.02 & 0.00 &  - & -  &  -  \\
H20-27 &  -  & 200.861764 & -42.958742 & 18.78$\pm$0.01 & 18.48$\pm$0.01 & 0.34 & -1.4 & r & 1.0 & 200.86174 & -42.958769 & 1.63$\pm$0.46 & 0.06$\pm$0.35 & 0.10$\pm$0.26 & 0.0 & 1.25 & 19.80 & 18.67 & 18.40 & 18.23 & 18.22 & 0.006 & 0.001 & 0.003 & 0.002 & 0.006 & 1.13 & 0.03 & 0.00 & 0.69 & 0.02 & 0.30 & 0.02 & 0.00 &  - & -  &  -  \\
H20-28 &  -  & 200.806883 & -43.182707 & 21.18$\pm$0.01 & 19.61$\pm$0.01 & 0.21 & 1.66 & r & 1.0 & 200.80683 & -43.182738 & -8.03$\pm$0.79 & 3.03$\pm$0.54 & 1.28$\pm$0.45 & 0.32 & 1.52 & 0.000 & 20.88 & 19.50 & 18.79 & 18.45 & 0.000 & 0.002 & 0.001 & 0.001 & 0.005 & 0.00 & 0.00 & 0.00 & 0.00 & 0.08 & 0.91 &  - & 0.00 &  - & -  &  -  \\
H20-29 &  -  & 201.029095 & -43.034494 & 18.89$\pm$0.01 & 18.40$\pm$0.01 & 0.33 & 0.94 & r & 1.0 & 201.02905 & -43.034516 & -4.73$\pm$0.41 & -2.79$\pm$0.34 & 0.07$\pm$0.27 & 0.0 & 1.26 & 20.13 & 18.82 & 18.44 & 18.29 & 18.28 & 0.008 & 0.001 & 0.000 & 0.000 & 0.007 & 1.44 & 0.03 & 0.00 & 0.79 & 0.02 & 0.40 & 0.02 & 0.00 &  - & -  &  -  \\
H20-30 &  -  & 201.048072 & -43.103887 & 18.98$\pm$0.01 & 18.35$\pm$0.01 & 0.64 & 1.51 & r & 1.0 & 201.04801 & -43.103906 & -7.22$\pm$0.45 & 0.03$\pm$0.37 & -0.03$\pm$0.30 & 0.59 & 1.29 & 20.38 & 18.87 & 18.37 & 18.16 & 18.07 & 0.008 & 0.001 & 0.000 & 0.000 & 0.003 & 1.76 & 0.16 & 0.00 & 0.89 & 0.66 & 0.63 & 0.02 & 0.00 &  - & -  &  -  \\
H20-31 &  -  & 200.804362 & -43.070461 & 20.74$\pm$0.01 & 20.22$\pm$0.01 & -0.4 & -0.8 & r & 1.0 & 200.80434 & -43.070496 & 3.31$\pm$2.14 & -1.03$\pm$1.13 & 0.10$\pm$0.84 & 1.28 & 1.42 & 21.81 & 20.47 & 19.37 & 19.56 & 15.75 & 0.023 & 0.003 & 0.001 & 0.002 & 0.004 & 2.16 & 3.47 & 0.24 & 0.90 & 0.28 & 0.35 & 0.02 & 0.00 &  - & -  &  -  \\
H20-32 &  -  & 200.941624 & -43.026274 & 21.40$\pm$0.02 & 19.93$\pm$0.01 & -2.0 & -1.7 & r & 1.0 & 200.94156 & -43.026302 & -18.40$\pm$1.30 & 2.75$\pm$0.97 & 0.75$\pm$0.84 & 1.81 & 1.43 & 0.000 & 21.21 & 19.87 & 19.19 & 18.92 & 0.000 & 0.003 & 0.001 & 0.001 & 0.012 & 0.00 & 0.00 & 0.00 & 0.36 & 0.80 & 0.56 &  - & 0.00 &  - & -  &  -  \\
H20-33 & H12\_399$^w$ & 200.858944 & -42.955117 & 19.96$\pm$0.01 & 19.49$\pm$0.01 & 16.56 & 19.73 & r & 0.0 &  - & - & - & - & - & - & - & - &  20.42 & 18.11 & 17.41 & 17.09 & 17.18 & 0.029 & 0.001 & 0.000 & 0.001 & 0.008 & 2.73 & 0.09 &  - & - & - & - & 0.02 & 0.00 &  - & -  &  w  \\
H20-34 &  -  & 200.857827 & -42.838555 & 19.68$\pm$0.01 & 18.28$\pm$0.01 & -2.1 & 0.53 & r & 1.0 & 200.85776 & -42.838589 & -10.05$\pm$0.44 & -1.88$\pm$0.33 & 0.40$\pm$0.24 & 0.0 & 1.37 & 22.33 & 19.47 & 18.15 & 17.61 & 17.37 & 0.039 & 0.001 & 0.000 & 0.000 & 0.002 & 3.89 & 0.63 & 0.00 & 0.10 & 0.02 & 0.98 & 0.02 & 0.00 &  - & -  &  -  \\
H20-35 &  -  & 200.878697 & -43.181095 & 19.77$\pm$0.01 & 19.32$\pm$0.01 & 0.87 & 0.92 & r & 1.0 & 200.87867 & -43.181135 & -3.00$\pm$0.79 & -4.77$\pm$0.50 & 0.90$\pm$0.39 & 0.0 & 1.28 & 20.80 & 19.69 & 19.35 & 19.20 & 19.15 & 0.014 & 0.001 & 0.000 & 0.001 & 0.008 & 1.17 & 0.05 & 0.00 & 0.02 & 0.02 & 0.28 & 0.02 & 0.00 &  - & -  &  -  \\
H20-36 &  -  & 200.967032 & -43.030028 & 19.79$\pm$0.01 & 18.46$\pm$0.01 & -0.6 & -0.3 & r & 1.0 & 200.96698 & -43.030057 & -6.49$\pm$0.42 & 0.67$\pm$0.37 & 1.05$\pm$0.36 & 0.0 & 1.36 & 22.50 & 19.61 & 18.40 & 17.92 & 17.68 & 0.049 & 0.001 & 0.000 & 0.000 & 0.006 & 3.84 & 0.59 & 0.00 & 0.00 & 0.02 & 0.94 & 0.02 & 0.00 &  - & -  &  -  \\
H20-37 &  -  & 200.803347 & -43.182398 & 19.32$\pm$0.01 & 18.38$\pm$0.01 & -0.3 & -0.1 & r & 1.0 & 200.80332 & -43.182429 & -3.62$\pm$0.47 & 3.71$\pm$0.42 & -0.21$\pm$0.35 & 0.92 & 1.32 & 21.51 & 19.17 & 18.33 & 17.98 & 17.86 & 0.017 & 0.001 & 0.001 & 0.001 & 0.003 & 2.88 & 0.32 & 0.00 & 0.54 & 0.97 & 0.80 & 0.02 & 0.00 &  - & -  &  -  \\
H20-38 &  -  & 200.912624 & -43.105774 & 21.55$\pm$0.02 & 20.95$\pm$0.03 & 0.91 & -0.6 & r & 1.0 &  - & - & - & - & - & - & - & - &  22.73 & 21.48 & 20.98 & 20.74 & 20.72 & 0.051 & 0.003 & 0.002 & 0.003 & 0.024 & 1.50 & 0.11 &  - & - & - & - & 0.02 & 0.00 &  - & -  &  -  \\
H20-39 &  -  & 200.852259 & -43.070318 & 20.70$\pm$0.01 & 19.17$\pm$0.01 & -1.1 & -0.7 & r & 1.0 & 200.85221 & -43.070354 & -2.76$\pm$0.57 & -1.07$\pm$0.42 & 0.69$\pm$0.33 & 0.70 & 1.43 & 23.20 & 20.49 & 19.07 & 18.18 & 17.78 & 0.080 & 0.002 & 0.000 & 0.000 & 0.002 & 3.85 & 1.15 & 0.00 & 0.03 & 0.53 & 0.92 & 0.02 & 0.00 &  - & -  &  -  \\
H20-40 & H12\_262$^w$ & 200.729137 & -43.179923 & 20.14$\pm$0.01 & 19.52$\pm$0.01 & 5.64 & 7.60 & r & 1.0 & 200.72913 & -43.179955 &  - &  - &  - & 12.75 & 2.70 & 21.43 & 19.96 & 19.36 & 19.07 & 18.94 & 0.031 & 0.002 & 0.001 & 0.001 & 0.008 & 1.77 & 0.26 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  -  &  w;y  \\
H20-41 &          165$^i$ & 201.025904 & -42.962377 & 20.96$\pm$0.01 & 20.06$\pm$0.01 & 15.48 & 21.36 & r & 0.0 &  - & - & - & - & - & - & - & - &  22.02 & 20.66 & 19.78 & 19.33 & 19.06 & 0.041 & 0.002 & 0.001 & 0.001 & 0.013 & 1.98 & 0.58 &  - & - & - & - & 0.02 & 0.00 &  - & -  &  i  \\
H20-43 &  -  & 200.656174 & -43.107494 & 20.98$\pm$0.01 & 20.03$\pm$0.01 & -0.6 & -0.1 & r & 1.0 & 200.65614 & -43.107515 & 1.01$\pm$1.39 & -0.39$\pm$1.05 & -0.46$\pm$0.74 & 0.75 & 1.15 & 23.13 & 20.86 & 20.01 & 19.69 & 19.55 & 0.066 & 0.002 & 0.001 & 0.001 & 0.011 & 2.81 & 0.29 & 0.72 & 0.53 & 0.14 & 0.05 & 0.02 & 0.00 &  - & -  &  -  \\
H20-44 &  -  & 200.836369 & -42.859684 & 18.88$\pm$0.01 & 18.22$\pm$0.01 & -0.2 & 0.71 & r & 1.0 & 200.83632 & -42.859713 & -5.64$\pm$0.42 & 0.07$\pm$0.31 & -0.14$\pm$0.23 & 0.0 & 1.24 & 20.26 & 18.76 & 18.27 & 18.07 & 18.02 & 0.008 & 0.001 & 0.000 & 0.000 & 0.006 & 1.71 & 0.09 & 0.00 & 0.53 & 0.02 & 0.27 & 0.02 & 0.00 &  - & -  &  -  \\
H20-45 &  -  & 200.990481 & -43.029881 & 21.25$\pm$0.01 & 19.53$\pm$0.01 & 1.54 & 0.83 & r & 1.0 & 200.99043 & -43.029908 & -1.08$\pm$0.77 & -1.01$\pm$0.62 & 0.38$\pm$0.51 & 0.77 & 1.58 & 0.000 & 20.75 & 19.30 & 18.35 & 17.87 & 0.000 & 0.002 & 0.001 & 0.000 & 0.007 & 0.00 & 0.00 & 0.10 & 0.45 & 0.39 & 0.98 &  - & 0.00 &  - & -  &  -  \\
H20-46 &  -  & 200.877236 & -43.069785 & 20.64$\pm$0.01 & 19.89$\pm$0.01 & -0.4 & -0.5 & r & 1.0 & 200.87718 & -43.069825 & -12.24$\pm$1.38 & -3.87$\pm$0.99 & 0.25$\pm$0.80 & 2.53 & 1.19 & 22.46 & 20.52 & 19.91 & 19.69 & 19.62 & 0.036 & 0.002 & 0.001 & 0.001 & 0.010 & 2.29 & 0.15 & 0.00 & 0.75 & 0.97 & 0.07 & 0.02 & 0.00 &  - & -  &  -  \\
H20-47 &  -  & 200.885437 & -42.925020 & 19.33$\pm$0.01 & 18.68$\pm$0.01 & 0.39 & -0.4 & r & 1.0 & 200.88540 & -42.925043 & -2.06$\pm$0.51 & 0.69$\pm$0.46 & 0.35$\pm$0.37 & 0.63 & 1.30 & 20.77 & 19.22 & 18.70 & 18.50 & 18.44 & 0.010 & 0.001 & 0.000 & 0.000 & 0.005 & 1.80 & 0.11 & 0.00 & 0.35 & 0.53 & 0.48 & 0.02 & 0.00 &  - & -  &  -  \\
H20-49 &  -  & 200.765712 & -42.889145 & 21.20$\pm$0.01 & 19.63$\pm$0.01 & -1.3 & -1.0 & r & 1.0 & 200.76563 & -42.889172 & -17.02$\pm$0.56 & 1.78$\pm$0.42 & 2.49$\pm$0.28 & 0.0 & 1.49 & 0.000 & 20.93 & 19.49 & 18.09 & 17.53 & 0.000 & 0.002 & 0.000 & 0.000 & 0.002 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.98 &  - & 0.00 &  - & -  &  -  \\
H20-50 &  -  & 201.029902 & -43.180537 & 20.46$\pm$0.01 & 20.06$\pm$0.01 & 1.03 & -0.1 & r & 1.0 & 201.02986 & -43.180560 & -6.43$\pm$1.78 & 1.87$\pm$1.44 & -0.82$\pm$0.96 & 0.58 & 1.44 & 21.47 & 20.41 & 20.08 & 19.93 & 19.89 & 0.020 & 0.002 & 0.001 & 0.001 & 0.013 & 1.13 & 0.05 & 0.00 & 0.39 & 0.09 & 0.45 & 0.02 & 0.00 &  - & -  &  -  \\
H20-51 &  -  & 200.619317 & -43.107309 & 21.33$\pm$0.01 & 20.71$\pm$0.02 & -0.3 & 1.81 & r & 1.0 & 200.61929 & -43.107328 &  - &  - &  - & 2.61 & 1.80 & 22.78 & 21.23 & 20.72 & 20.54 & 20.51 & 0.044 & 0.003 & 0.002 & 0.002 & 0.019 & 1.75 & 0.05 &  - &  - & 0.50 & 0.68 & 0.02 & 0.00 & gold &  -  &  -  \\
H20-52 &  -  & 201.009268 & -42.996721 & 20.15$\pm$0.01 & 19.36$\pm$0.01 & 0.55 & -1.0 & r & 1.0 & 201.00923 & -42.996740 & -1.31$\pm$1.02 & 1.59$\pm$0.76 & -0.61$\pm$0.62 & 1.67 & 1.35 & 21.65 & 19.99 & 19.37 & 19.12 & 19.04 & 0.022 & 0.001 & 0.000 & 0.001 & 0.008 & 2.02 & 0.20 & 0.06 & 0.32 & 0.94 & 0.49 & 0.02 & 0.00 &  - & -  &  -  \\
\hline
\end{tabular}
  
\begin{tablenotes}
\small
\item Note on column names: $\mu_{\alpha*} \equiv \mu_\alpha \cos \delta$ is the proper motion in right ascension direction; $\mu_\delta$ is the proper motion in declination direction; $\varpi$ is the absolute stellar parallax; $\mathscr{L}$ denotes likelihood values
\item *see Table \ref{table:confirmed_short} for annotation reference
\end{tablenotes}
\label{table:all_table}
\end{sidewaystable}


==> table_cands.tex <==
\begin{sidewaystable}
\tiny
\centering
\caption{Candidate GCs around NGC~5128}
\renewcommand{\tabcolsep}{1.05mm}
  
\begin{tabular}{c c c c c c c c c c c c c c c c c c c c c c c c}
\hline \hline
ID & Discovery & R.A. & Decl.   &  g  & r  & $C_{3-6}$ &  Gaia G & $\mu_{\alpha*}$ &  $\mu_{\delta}$  & $\varpi$ &  AEN   &  BR$_{\rm exc.}$ &  $(u-r)_0$  & $(r-z)_0$ &  $\mu$  & $\varpi$  &  AEN  &  BRE  & Color & Total &  data  &  conf? &    refs.  \\
(H20) &  ID*  & (J2000) & (J2000) & (mag) & (mag) &   &  (mag) &  (mas/yr) &  (mas/yr) & (mas) &   &   & (mag) & (mag) &  $\mathscr{L}$ & $\mathscr{L}$  & $\mathscr{L}$  & $\mathscr{L}$  & $\mathscr{L}$  & $\mathscr{L}$  & group &     &       \\
\hline
H20-40 & H12\_262$^v$ & 200.729137 & -43.179923 & 20.14$\pm$0.01 & 19.52$\pm$0.01 & 7.60 & 20.23 &  - &  - &  - & 12.75 & 2.70 & 1.77 & 0.26 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  &  v;x  \\
H20-130 & H12\_222$^v$ & 200.829280 & -42.836771 & 20.00$\pm$0.01 & 19.14$\pm$0.01 & 5.43 & 19.67 &  - &  - &  - & 7.73 & 2.20 & 2.33 & 0.51 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  &  v;x  \\
H20-352 & GC0010$^m$ & 200.994863 & -43.026354 & 19.47$\pm$0.01 & 18.44$\pm$0.01 & 9.11 & 19.30 &  - &  - &  - & 10.01 & 2.74 & 2.44 & 0.56 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  y &  m;n;r;x  \\
H20-612 & GC0563$^r$ & 200.937603 & -43.019830 & 19.67$\pm$0.01 & 18.85$\pm$0.01 & 5.39 & 19.54 &  - &  - &  - & 7.83 & 2.35 & 2.31 & 0.45 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  y &  r;x  \\
H20-3793 & C40$^e$ & 200.926424 & -43.160459 & 19.37$\pm$0.01 & 18.64$\pm$0.01 & 8.48 & 19.54 &  - &  - &  - & 15.28 & 2.82 & 2.04 & 0.31 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  y &  e;f;h;j;m;n;x  \\
H20-29570 &  & 202.060207 & -43.330839 & 20.49$\pm$0.01 & 19.65$\pm$0.01 & 2.17 & 20.30 &  - &  - &  - & 13.40 & 1.92 & 1.94 & 0.33 &  - &  - & 1.00 & 0.97 & 1.00 & 0.96 & gold &  &   \\
H20-30857 &  & 201.674264 & -43.272770 & 19.80$\pm$0.01 & 19.00$\pm$0.01 & 4.50 & 19.38 &  - &  - &  - & 4.95 & 1.57 & 2.06 & 0.28 &  - &  - & 1.00 & 0.98 & 0.99 & 0.97 & gold &  &   \\
H20-86420 &  & 202.120380 & -42.763852 & 20.06$\pm$0.01 & 19.05$\pm$0.01 & 6.23 & 20.14 &  - &  - &  - & 19.65 & 3.78 & 2.51 & 0.66 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  &   \\
H20-87646 &  & 202.281954 & -43.005488 & 19.75$\pm$0.01 & 18.68$\pm$0.01 & 5.89 & 19.95 &  - &  - &  - & 15.54 & 3.61 & 2.38 & 0.62 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  &   \\
H20-91425 &  & 202.507473 & -42.876689 & 18.57$\pm$0.01 & 17.88$\pm$0.01 & 5.87 & 18.24 &  - &  - &  - & 8.26 & 1.59 & 1.88 & 0.24 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  &   \\
H20-84006 & pff\_gc-102$^f$ & 202.076936 & -42.553438 & 19.66$\pm$0.01 & 19.03$\pm$0.01 & 4.00 & 19.68 & -13.34$\pm$2.70 & -1.85$\pm$1.67 & -0.04$\pm$1.18 & 6.48 & 2.22 & 1.86 & 0.29 & 1.00 & 0.96 & 1.00 & 1.00 & 1.00 & 0.96 & gold &  y &  f;h;m;n;x  \\
H20-126 &  & 200.854929 & -43.179955 & 21.38$\pm$0.01 & 20.84$\pm$0.02 & 1.39 &  - & - & - & - & - & - &  1.68 & 0.23 &  -  & -  & -  & -  & 0.99 & 0.91 & silver &  &   \\
H20-349 &  & 200.645763 & -43.176665 & 21.53$\pm$0.02 & 20.29$\pm$0.01 & 14.13 &  - & - & - & - & - & - &  2.71 & 0.67 &  -  & -  & -  & -  & 0.93 & 0.93 & silver &  &   \\
H20-384 & H12\_760$^v$ & 200.633346 & -42.955045 & 21.67$\pm$0.02 & 21.03$\pm$0.03 & 16.67 &  - & - & - & - & - & - &  1.80 & 0.31 &  -  & -  & -  & -  & 0.99 & 0.99 & silver &  &  v;x  \\
H20-413 &  & 200.736899 & -43.053167 & 22.05$\pm$0.03 & 20.42$\pm$0.01 & 10.55 & 20.47 &  - &  - &  - & 9.20 & 2.49 &   - &  - &   - &  - & 1.00 & 0.99 &  - & 0.99 & silver &  &   \\
H20-506 &  & 200.662918 & -43.138449 & 21.52$\pm$0.02 & 19.99$\pm$0.01 & 5.02 & 20.25 &  - &  - &  - & 7.38 & 2.41 &   - &  - &   - &  - & 1.00 & 0.99 &  - & 0.99 & silver &  &   \\
H20-531 &  & 200.614325 & -43.137770 & 21.97$\pm$0.03 & 20.92$\pm$0.02 & 1.16 & 21.03 &  - &  - &  - & 4.68 &  - &   - &  - &   - &  - & 1.00 &  - &  - & 0.87 & silver &  &   \\
H20-879 & H12\_518$^v$ & 201.053635 & -43.204602 & 21.42$\pm$0.01 & 20.60$\pm$0.02 & 15.14 &  - & - & - & - & - & - &  1.89 & 0.35 &  -  & -  & -  & -  & 0.96 & 0.96 & silver &  &  v;x  \\
H20-903 & H12\_453$^v$ & 201.035190 & -43.204626 & 20.99$\pm$0.01 & 20.38$\pm$0.01 & 8.55 &  - & - & - & - & - & - &  1.64 & 0.26 &  -  & -  & -  & -  & 0.99 & 0.99 & silver &  &  v;x  \\
H20-940 & GC0484$^r$ & 201.045773 & -43.204387 & 21.66$\pm$0.02 & 20.74$\pm$0.02 & 8.10 &  - & - & - & - & - & - &  2.59 & 0.63 &  -  & -  & -  & -  & 0.85 & 0.85 & silver &  y &  r;x  \\
H20-1135 &  & 200.809488 & -43.190368 & 21.87$\pm$0.03 & 20.62$\pm$0.02 & 1.29 & 20.39 &  - &  - &  - & 5.76 &  - &   - &  - &   - &  - & 0.99 &  - &  - & 0.90 & silver &  &   \\
H20-0 & KKs55-02$^aa$ & . & 0.0000000 & 0.000$\pm$0.01 & 0.000$\pm$0.01 &   & 0.000 & 0$\pm$0 & 0$\pm$0 & 0$\pm$0 & 0.0 & 0.0 &   - &  - &  0.00 & 0.00 & 0.00 & 0.00 &  - & 0.00 &  &  &   \\
H20-84 &  & 200.994368 & -43.180090 & 22.26$\pm$0.04 & 21.08$\pm$0.03 & 2.41 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.99 & bronze &  &   \\
H20-190 &  & 200.826018 & -43.180492 & 21.84$\pm$0.02 & 21.07$\pm$0.03 & 17.69 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 1.00 & bronze &  &   \\
H20-224 &  & 200.797217 & -42.851973 & 21.94$\pm$0.03 & 20.58$\pm$0.02 & 9.24 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 1.00 & bronze &  &   \\
H20-572 &  & 200.962802 & -43.175061 & 22.04$\pm$0.03 & 20.94$\pm$0.02 & 2.96 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.99 & bronze &  &   \\
H20-743 &  & 201.044873 & -43.027365 & 22.19$\pm$0.03 & 21.44$\pm$0.04 & 20.50 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 1.00 & bronze &  &   \\
H20-820 &  & 200.715999 & -42.982224 & 22.17$\pm$0.04 & 20.60$\pm$0.02 & 7.92 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 1.00 & bronze &  &   \\
H20-932 &  & 200.924826 & -43.204435 & 22.55$\pm$0.05 & 21.84$\pm$0.06 & 8.96 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 1.00 & bronze &  &   \\
H20-964 &  & 200.909000 & -43.201325 & 23.43$\pm$0.12 & 21.73$\pm$0.05 & 2.35 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.99 & bronze &  &   \\
H20-1078 &  & 200.896149 & -43.193416 & 22.08$\pm$0.03 & 21.55$\pm$0.05 & 17.51 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 1.00 & bronze &  &   \\
H20-1114 &  & 200.685539 & -43.190830 & 22.99$\pm$0.08 & 21.19$\pm$0.03 & 10.78 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 1.00 & bronze &  &   \\
H20-40 & H12\_262$^v$ & 200.729137 & -43.179923 & 20.14$\pm$0.01 & 19.52$\pm$0.01 & 7.60 & 20.23 &  - &  - &  - & 12.75 & 2.70 & 1.77 & 0.26 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  &  v;x  \\
H20-130 & H12\_222$^v$ & 200.829280 & -42.836771 & 20.00$\pm$0.01 & 19.14$\pm$0.01 & 5.43 & 19.67 &  - &  - &  - & 7.73 & 2.20 & 2.33 & 0.51 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  &  v;x  \\
H20-352 & GC0010$^m$ & 200.994863 & -43.026354 & 19.47$\pm$0.01 & 18.44$\pm$0.01 & 9.11 & 19.30 &  - &  - &  - & 10.01 & 2.74 & 2.44 & 0.56 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  y &  m;n;r;x  \\
H20-384 & H12\_760$^v$ & 200.633346 & -42.955045 & 21.67$\pm$0.02 & 21.03$\pm$0.03 & 16.67 &  - & - & - & - & - & - &  1.80 & 0.31 &  -  & -  & -  & -  & 0.99 & 0.99 & silver &  &  v;x  \\
H20-612 & GC0563$^r$ & 200.937603 & -43.019830 & 19.67$\pm$0.01 & 18.85$\pm$0.01 & 5.39 & 19.54 &  - &  - &  - & 7.83 & 2.35 & 2.31 & 0.45 &  - &  - & 1.00 & 1.00 & 1.00 & 1.00 & gold &  y &  r;x  \\
H20-879 & H12\_518$^v$ & 201.053635 & -43.204602 & 21.42$\pm$0.01 & 20.60$\pm$0.02 & 15.14 &  - & - & - & - & - & - &  1.89 & 0.35 &  -  & -  & -  & -  & 0.96 & 0.96 & silver &  &  v;x  \\
H20-903 & H12\_453$^v$ & 201.035190 & -43.204626 & 20.99$\pm$0.01 & 20.38$\pm$0.01 & 8.55 &  - & - & - & - & - & - &  1.64 & 0.26 &  -  & -  & -  & -  & 0.99 & 0.99 & silver &  &  v;x  \\
H20-940 & GC0484$^r$ & 201.045773 & -43.204387 & 21.66$\pm$0.02 & 20.74$\pm$0.02 & 8.10 &  - & - & - & - & - & - &  2.59 & 0.63 &  -  & -  & -  & -  & 0.85 & 0.85 & silver &  y &  r;x  \\
H20-1152 & VHH81-01$^a$ & 200.934075 & -43.186591 & 18.12$\pm$0.01 & 17.38$\pm$0.01 & 21.36 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 1.00 & bronze &  y &  a;f;h;m;n;r;t;w;x  \\
H20-1389 & H12\_603$^v$ & 200.960370 & -42.985642 & 21.68$\pm$0.02 & 20.84$\pm$0.02 & 14.66 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 1.00 & bronze &  &  v  \\
H20-133 &  & 200.999930 & -43.212001 & 23.09$\pm$0.09 & 21.57$\pm$0.05 & 1.97 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.97 & copper &  &   \\
H20-211 &  & 200.672232 & -43.088388 & 21.58$\pm$0.02 & 20.82$\pm$0.02 & 1.61 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.94 & copper &  &   \\
H20-442 &  & 200.705245 & -43.052931 & 22.01$\pm$0.03 & 20.98$\pm$0.03 & 1.57 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.94 & copper &  &   \\
H20-815 &  & 200.998736 & -43.213352 & 23.37$\pm$0.12 & 21.78$\pm$0.06 & 1.27 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.89 & copper &  &   \\
H20-851 &  & 200.846811 & -43.209938 & 22.25$\pm$0.04 & 21.71$\pm$0.06 & 1.95 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.97 & copper &  &   \\
H20-853 &  & 200.777250 & -43.209860 & 23.33$\pm$0.11 & 21.84$\pm$0.06 & 1.54 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.93 & copper &  &   \\
H20-869 &  & 200.683329 & -43.208821 & 23.58$\pm$0.14 & 21.96$\pm$0.07 & 1.81 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.96 & copper &  &   \\
H20-938 &  & 200.804536 & -43.203453 & 23.02$\pm$0.08 & 21.63$\pm$0.05 & 1.22 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.88 & copper &  &   \\
H20-953 &  & 200.627696 & -43.202318 & 22.14$\pm$0.03 & 21.70$\pm$0.06 & 1.59 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.94 & copper &  &   \\
H20-956 &  & 200.969001 & -43.202241 & 23.34$\pm$0.11 & 21.91$\pm$0.07 & 1.51 &  - & - & - & - & - & - &    - &  - &   -  & -  & -  & -  &  - & 0.93 & copper &  &   \\
\hline
\end{tabular}
  
\begin{tablenotes}
\small
\item Note on column names: $\mu_{\alpha*} \equiv \mu_\alpha \cos \delta$ is the proper motion in right ascension direction; $\mu_\delta$ is the proper motion in declination direction; $\varpi$ is the absolute stellar parallax; $\mathscr{L}$ denotes likelihood values
\item *see Table \ref{table:confirmed_short} for annotation reference
\end{tablenotes}
\label{table:cands_table}
\end{sidewaystable}


==> table_confirmed.tex <==
\begin{table*}[ht]
\tiny
\centering
\caption{Confirmed GCs in NGC~5128}
\begin{tabular}{c c c c c c c c c c}
\hline \hline
ID & Discovery ID & other IDs & R.A. & Decl.   & v$_r$         & v$_r$ Ref.** & $g$  &  $r$  & Notes  \\
(H20) &           &        & (J2000) & (J2000) & (km s$^{-1}$) &                & (mag) & (mag) &    \\
\hline

     & KK197-01$^z$ & KK197-01$^o$ & 200.49928 & -42.534884 & 636 $\pm$ 16 & z & 23.03 & 22.48 &   \\
H20_000021 & GC0010$^m$ & AAT101906$^n$;GC0010$^r$;T17-1050$^x$ & 200.99486 & -43.026354 & 496 $\pm$ 21 & r & 19.47 & 18.44 & 1 \\
H20_000044 & GC0563$^r$ & T17-1014$^x$ & 200.93760 & -43.019830 & 533 $\pm$ 35 & r & 19.67 & 18.85 & 1 \\
H20_000066 & GC0484$^r$ & T17-1092$^x$ & 201.04577 & -43.204387 & 498 $\pm$ 22 & r & 21.66 & 20.74 &   \\
     & VHH81-01$^a$ & HGHH-01$^f$;C1$^g$;GC0005$^m$;HGHH-01$^n$;GC0005$^t$;GC0005$^r$;0005$^w$;T17-1010$^x$ & 200.93408 & -43.186591 & 642 $\pm$ 1 & r & 18.12 & 17.38 &   \\
H20_000270 & GC0480$^r$ & T17-1022$^x$ & 200.96041 & -43.195503 & 646 $\pm$ 61 & r & 21.91 & 21.07 &   \\
H20_000283 & C40$^e$ & HGHH-40$^f$;C40$^g$;N1$^k$;GC0004$^m$;HGHH-40$^n$;T17-1008$^x$ & 200.92642 & -43.160459 & 443 $\pm$ 48 & n & 19.37 & 18.64 &   \\
H20_000424 & GC0018$^m$ & AAT305341$^n$;GC0018$^r$;T17-1091$^x$ & 201.04568 & -43.214673 & 439 $\pm$ 118 & r & 21.05 & 20.16 &   \\
H20_000425 & GC0564$^r$ & T17-1017$^x$ & 200.94762 & -43.071602 & 357 $\pm$ 66 & r & 21.25 & 20.27 &   \\
H20_000457 & GC0512$^r$ & T17-1514$^x$ & 201.32892 & -42.651050 & 631 $\pm$ 31 & r & 20.51 & 19.88 &   \\
     & GC0509$^r$ & T17-1461$^x$ & 201.30706 & -42.675718 & 306 $\pm$ 35 & r & 21.62 & 21.00 &   \\
H20_000503 & GC0514$^r$ & T17-1530$^x$ & 201.33646 & -42.696438 & 518 $\pm$ 19 & r & 20.84 & 20.08 & 1 \\
     & GC0508$^r$ & T17-1462$^x$ & 201.30708 & -42.793576 & 326 $\pm$ 71 & r & 22.24 & 21.63 &   \\
     & GC0012 & AAT102120;T17-1054 & 200.99837 & -42.922017 & 293 $\pm$ 83 & m & 19.92 & 19.35 & 1 \\
     & pff\_gc-004 & GC0015;PFF-gc004;T17-1061 & 201.01556 & -43.598156 & 634 $\pm$ 71 & m & 19.95 & 19.39 & 1 \\
     & C114 & GC0043;GC043;T17-1204 & 201.16863 & -42.893092 &   &    &       &       &   \\
     & GC0052 & AAT109711;GC052;AAT109711;0052;T17-1227 & 201.18893 & -42.992625 & 276 $\pm$ 59 & m & 19.15 & 18.89 & 1 \\
     & GC575 & GC0575;T17-1240 & 201.19923 & -43.145415 & 353 $\pm$ 29 & p & 19.83 & 19.52 & 1 \\
     & HGHH-G302 & G302;HGHH-G302;G302;GC0070;GC070;G302;GC0070;T17-1273 & 201.22200 & -43.076318 & 485 $\pm$ 23 & p & 19.19 & 18.66 & 1 \\
     & C116 & GC0079;GC079;T17-1296 & 201.23100 & -43.166203 &   &    &       &       &   \\
     & HGHH-G279 & HGHH-G279;G279;GC0084;HGHH-G279;G279;0084;T17-1304 & 201.23441 & -43.056503 & 338 $\pm$ 54 & m & 19.22 & 19.10 & 1 \\
     & GC0580 & T17-1311 & 201.23791 & -42.648595 & 170 $\pm$ 45 & p & 18.78 & 18.46 &   \\
     & C121 & GC0092;T17-1325 & 201.24342 & -43.139222 &   &    &       &       &   \\
     & C122 & GC0094;T17-1332 & 201.24588 & -43.139278 &   &    &       &       &   \\
     & pff\_gc-027 & PFF027;GC0098;PFF-gc027;GC098;pff\_gc-027;GC0098;0098;T17-1343 & 201.25263 & -43.091744 & 503 $\pm$ 21 & p & 19.83 & 19.13 & 1 \\
     & C126 & GC0100;T17-1346 & 201.25379 & -43.154028 &   &    &       &       &   \\
     & GC582 & GC0582;T17-1349 & 201.25510 & -43.067093 & 539 $\pm$ 28 & p & 20.72 & 19.96 & 1 \\
     & GC498 & GC0498;T17-1351 & 201.25566 & -43.096247 & 472 $\pm$ 36 & p & 21.17 & 20.42 & 1 \\
     & GC499 & GC0499;T17-1359 & 201.25759 & -43.063355 & 600 $\pm$ 35 & p & 21.30 & 20.59 &   \\
     & GC0116 & AAT112752;GC116;AAT112752;T17-1381 & 201.26721 & -43.005449 & 733 $\pm$ 54 & o & 19.28 & 18.75 &   \\
     & GC457 & GC0457;GC0457;T17-1403 & 201.27845 & -42.958920 & 587 $\pm$ 25 & p & 20.24 & 19.50 & 1 \\
     & GC424 & LDSS2-20871;GC0424;T17-1404 & 201.27870 & -43.044493 & 354 $\pm$ 14 & p & 19.66 & 19.13 &   \\
     &           18 & WHH-8;GC0129;GC129;WHH-8;GC0129;0129;T17-1412 & 201.28183 & -43.020890 & 689 $\pm$ 11 & p & 18.24 & 17.50 &   \\
     & HGHH-G329 & HGHH-G329;G329;GC0136;HGHH-G329;GC136;T17-1428 & 201.29243 & -43.035203 & 485 $\pm$ 34 & m & 19.99 & 19.11 &   \\
     & GC505 & GC0505;T17-1450 & 201.30291 & -43.032175 & 578 $\pm$ 20 & p & 20.29 & 19.58 &   \\
     & GC0509 & T17-1461 & 201.30706 & -42.675718 & 306 $\pm$ 35 & p & 21.20 & 20.71 & 1 \\
     & GC0508 & T17-1462 & 201.30708 & -42.793576 & 326 $\pm$ 71 & p & 21.84 & 21.35 & 1 \\
     & GC587 & GC0587;T17-1523 & 201.33361 & -43.052768 & 278 $\pm$ 37 & p & 20.29 & 19.59 &   \\
     & GC429 & GC0429;0429;T17-1540 & 201.34536 & -43.136148 & 146 $\pm$ 110 & p & 19.16 & 18.19 &   \\
     & GC0221 & AAT205071;T17-1600 & 201.37813 & -42.504435 & 288 $\pm$ 61 & m & 18.81 & 18.41 & 1 \\
     & HGHH-G359 & HGHH-G359;G359;GC0230;HGHH-G359;G359;GC0230;T17-1614 & 201.38509 & -42.980563 & 489 $\pm$ 14 & p & 18.93 & 18.25 &   \\
     &           66 & K131;GC0233;K-131;GC233;K-131;T17-1618 & 201.38699 & -43.074742 & 607 $\pm$ 23 & o & 19.48 & 18.74 &   \\
     & f2.GC-17 & GC432;GC0432;0432;T17-1627 & 201.39200 & -43.179369 & 396 $\pm$ 84 & p &       &       & 1 \\
     & HGHH-G206 & HGHH-G206;G206;GC0238;G206;T17-1628 & 201.39209 & -42.983485 & 716 $\pm$ 34 & o & 19.17 & 18.50 &   \\
     &           35 & WHH-22;WHH22;GC0248;GC248;WHH-22;T17-1648 & 201.39712 & -43.091389 & 599 $\pm$ 17 & o &       &       &   \\
     & MAGJM-08 &          312;GC0249;K-147;MAGJM-08;T17-1649 & 201.39792 & -42.993090 & 730 $\pm$ 31 & o & 19.57 & 18.86 &   \\
     & R213 & GC0251;GC251;T17-1651 & 201.39970 & -43.124426 & 532 $\pm$ 52 & l & 21.10 & 20.36 & 1 \\
     & GC0433 & T17-1653 & 201.40052 & -42.937939 & 575 $\pm$ 56 & p & 21.73 & 21.58 & 1 \\
     & LDSS2-14627 & GC0436;T17-1700 & 201.42383 & -42.975434 & 456 $\pm$ 10 & p & 19.14 & 18.47 &   \\
     & HGHH-G378 & HGHH-G378;GC0293;HGHH-G378;T17-1741 & 201.44217 & -43.023017 & 515 $\pm$ 43 & m & 19.76 & 19.03 &   \\
     & GC439 & GC0439;0439;T17-1753 & 201.44582 & -42.924969 & 700 $\pm$ 48 & p &       &       & 1 \\
     & C168 & GC0302;GC0302;T17-1763 & 201.45192 & -43.120139 & 650 $\pm$ 28 & p &       &       & 1 \\
     & HGHH-G251 & HGHH-G251;G251;GC0303;HGHH-G251;G251;GC0303;T17-1764 & 201.45226 & -42.961407 & 592 $\pm$ 8 & p & 19.01 & 18.33 & 1 \\
     & GC0535 & T17-1833 & 201.48250 & -42.861056 & 557 $\pm$ 93 & p &       &       & 1 \\
     & C170 & GC0332;T17-1838 & 201.48391 & -42.936922 &   &    & 22.57 & 22.16 &   \\
     & GC0333 & AAT121367;GC333;GC0333;0333;T17-1841 & 201.48435 & -43.025782 & 438 $\pm$ 80 & p & 20.14 & 19.78 & 1 \\
     & GC0538 & T17-1848 & 201.48658 & -42.880111 & 511 $\pm$ 11 & p &       &       & 1 \\
     & GC0335 & AAT329209;T17-1852 & 201.48857 & -43.685817 & 601 $\pm$ 66 & m & 19.90 & 19.36 & 1 \\
     & GC541 & GC0541;T17-1888 & 201.50562 & -43.042999 & 471 $\pm$ 30 & p & 21.08 & 20.39 & 1 \\
     &          250 & C177;GC0359;T17-1902 & 201.51333 & -42.908361 &   &    &       &       &   \\
     & GC0363 & AAT122794;T17-1914 & 201.51955 & -42.793058 & 336 $\pm$ 160 & m & 20.16 & 19.39 & 1 \\
     & C105 & C105;GC0364;T17-1917 & 201.52100 & -42.926750 &   &    &       &       &   \\
     & GC444 & GC0444;T17-1993 & 201.58596 & -42.896091 & 271 $\pm$ 64 & p & 20.58 & 20.12 & 1 \\
     & pff\_gc-091 & PFF091;GC0389;PFF-gc091;T17-1998 & 201.58799 & -43.706809 & 669 $\pm$ 57 & m & 19.30 & 18.73 & 1 \\
     & GC0604 & T17-2042 & 201.62812 & -42.754139 & 222 $\pm$ 34 & p &       &       &   \\
     & R105 & GC0403;R105;GC0403;T17-2051 & 201.63979 & -42.850196 & 534 $\pm$ 33 & p & 19.90 & 19.39 & 1 \\
     & GC552 & GC0552;T17-2062 & 201.65700 & -43.178083 & 548 $\pm$ 33 & p &       &       & 1 \\
     & HHH86-39 & C39;C39;GC0406;HHH86-39;GC406;T17-2078 & 201.67487 & -43.129149 & 271 $\pm$ 20 & l &       &       & 1 \\
     & GC557 & GC0557;T17-2104 & 201.71200 & -43.122378 & 372 $\pm$ 42 & p & 21.13 & 20.54 & 1 \\
     & GC0606 &  & 201.30167 & -43.587622 &   &    &       &       &   \\
     & GC0607 &  & 201.33242 & -43.578425 &   &    & 22.36 & 21.81 &   \\
     & HCH99-21 & HCH99-21 & 201.39333 & -43.058333 & 662 $\pm$ 1 & k &       &       &   \\
H20-1 & GC0018 & AAT305341;GC0018;T17-1091 & 201.04568 & -43.214673 & 439 $\pm$ 118 & p & 20.61 & 19.86 & 1 \\
H20-8 & GC0484 & T17-1092 & 201.04577 & -43.204387 & 498 $\pm$ 22 & p & 21.22 & 20.44 & 1 \\
H20-23 & GC0480 & T17-1022 & 200.96041 & -43.195503 & 646 $\pm$ 61 & p & 21.46 & 20.76 & 1 \\
H20-38 & VHH81-01 & HGHH-01;C1;HGHH92-C1;GC0005;HGHH-01;GC0005;0005;T17-1010 & 200.93408 & -43.186591 & 642 $\pm$ 1 & p & 17.67 & 17.07 & 1 \\
H20-67 & C40 & HGHH-40;C40;N1;GC0004;HGHH-40;T17-1008 & 200.92642 & -43.160459 & 443 $\pm$ 48 & m & 18.93 & 18.33 & 1 \\
H20-115 & GC0487 & T17-1124 & 201.08589 & -43.135543 & 576 $\pm$ 16 & p & 20.60 & 19.80 & 1 \\
H20-119 & pff\_gc-006 & PFF006;N7;GC0022;PFF-gc006;GC0022;T17-1137 & 201.09876 & -43.131152 & 613 $\pm$ 16 & p & 19.15 & 18.68 & 1 \\
H20-161 & GC0485 & T17-1103 & 201.05736 & -43.092596 & 388 $\pm$ 20 & p & 20.72 & 19.90 & 1 \\
H20-197 & GC0564 & T17-1017 & 200.94762 & -43.071602 & 357 $\pm$ 66 & p & 20.83 & 19.98 & 1 \\
H20-242 &           22 & WHH-1;GC0021;HH-096;GC0021;T17-1128 & 201.08922 & -43.043615 & 596 $\pm$ 17 & p & 18.09 & 17.45 & 1 \\
H20-284 & GC0010 & AAT101906;GC0010;T17-1050 & 200.99486 & -43.026354 & 496 $\pm$ 21 & p & 19.05 & 18.16 & 1 \\
H20-300 & GC0563 & T17-1014 & 200.93760 & -43.019830 & 533 $\pm$ 35 & p & 19.25 & 18.56 & 1 \\
H20-497 & GC0486 & T17-1118 & 201.08108 & -42.908751 & 554 $\pm$ 11 & p & 19.57 & 18.88 & 1 \\
H20-499 & pff\_gc-007 & PFF007;GC0024;PFF-gc007;GC0024;T17-1139 & 201.10064 & -42.905694 & 616 $\pm$ 25 & p & 20.28 & 19.50 & 1 \\
H20-610 & GC417 & GC0417;0417;T17-1213 & 201.17667 & -42.863637 & 634 $\pm$ 26 & p & 19.55 & 19.21 & 1 \\
H20-629 & GC0567 & T17-1122 & 201.08215 & -42.845484 & 189 $\pm$ 34 & p & 20.20 & 19.51 &   \\
H20-651 &           65 & WHH-13;GC0189;HH-090;GC0189;T17-1532 & 201.33885 & -42.821654 & 450 $\pm$ 15 & p & 19.38 & 18.76 & 1 \\
H20-652 & pff\_gc-048 & PFF048;GC0163;PFF-gc048;T17-1479 & 201.31583 & -42.820830 & 483 $\pm$ 116 & m & 19.90 & 19.43 & 1 \\
H20-658 & HHH86-28 & C28;GC0019;HHH86-28;T17-1110 & 201.07525 & -42.816931 & 499 $\pm$ 48 & m & 18.44 & 17.90 & 1 \\
H20-661 & pff\_gc-023 & PFF023;PFF023;GC0076;PFF-gc023;GC076;GC0076;T17-1286 & 201.22729 & -42.816263 & 439 $\pm$ 26 & p & 19.51 & 19.01 & 1 \\
H20-665 & GC0516 & T17-1545 & 201.34718 & -42.813327 & 527 $\pm$ 11 & p & 19.69 & 19.21 & 1 \\
H20-686 & GC0511 & T17-1507 & 201.32630 & -42.797940 & 487 $\pm$ 39 & p & 21.39 & 20.75 & 1 \\
H20-719 &           32 & GC0003;HH-080;T17-1002 & 200.90970 & -42.773027 & 497 $\pm$ 33 & m & 18.39 & 17.90 & 1 \\
H20-723 & GC0501 & T17-1399 & 201.27561 & -42.771849 & 564 $\pm$ 71 & p & 20.69 & 20.05 & 1 \\
H20-764 & HHH86-14 & C14;C14;C14;GC0139;HHH86-14;T17-1432 & 201.29373 & -42.747983 & 723 $\pm$ 41 & m & 18.03 & 17.45 & 1 \\
H20-824 & pff\_gc-026 & PFF026;GC0093;PFF-gc026;T17-1326 & 201.24355 & -42.714810 & 580 $\pm$ 114 & m & 19.47 & 19.05 & 1 \\
H20-859 & GC0514 & T17-1530 & 201.33646 & -42.696438 & 518 $\pm$ 19 & p & 20.43 & 19.80 & 1 \\
H20-940 & GC0512 & T17-1514 & 201.32892 & -42.651050 & 631 $\pm$ 31 & p & 20.09 & 19.59 & 1 \\
H20-1329 & R111 & GC0376;R111;GC0376;T17-1952 & 201.54050 & -42.841508 & 716 $\pm$ 48 & p & 20.56 & 20.01 & 1 \\
H20-1370 & GC0540 & T17-1877 & 201.50272 & -42.819277 & 609 $\pm$ 46 & p & 21.68 & 21.07 & 1 \\
H20-1376 & pff\_gc-081 & PFF081;GC0346;PFF-gc081;T17-1874 & 201.50069 & -42.816835 & 308 $\pm$ 61 & m & 19.23 & 18.83 & 1 \\
H20-1384 & GC0596 & T17-1866 & 201.49740 & -42.814466 & 319 $\pm$ 19 & p & 20.23 & 19.80 & 1 \\
H20-1388 & R107 & GC0388;R107;GC0388;T17-1996 & 201.58798 & -42.811374 & 430 $\pm$ 23 & p & 19.79 & 19.18 & 1 \\
H20-1395 & HHH86-26 & C26;C26;GC0381;HHH86-26;GC0381;T17-1973 & 201.56363 & -42.808137 & 377 $\pm$ 11 & p & 18.22 & 17.54 & 1 \\
H20-1405 & pff\_gc-055 & PFF055;GC0220;PFF-gc055;GC0220;T17-1599 & 201.37807 & -42.803690 & 484 $\pm$ 47 & p & 19.75 & 19.44 & 1 \\
H20-1425 & GC0539 & T17-1850 & 201.48840 & -42.795707 & 534 $\pm$ 31 & p & 20.27 & 19.77 & 1 \\
H20-1459 & pff\_gc-093 & PFF093;GC0394;PFF-gc093;GC0394;T17-2006 & 201.59438 & -42.780474 & 575 $\pm$ 41 & p & 19.50 & 19.16 & 1 \\
H20-1470 & GC0536 & T17-1836 & 201.48349 & -42.773898 & 448 $\pm$ 39 & p & 20.40 & 20.28 & 1 \\
H20-1485 & C27 & GC0404;GC0404;T17-2064 & 201.66045 & -42.762675 & 627 $\pm$ 21 & p & 18.47 & 18.13 & 1 \\
H20-1528 & GC0525 & T17-1661 & 201.40498 & -42.723248 & 551 $\pm$ 41 & p & 21.14 & 20.51 & 1 \\
H20-1589 & GC0526 & T17-1663 & 201.40690 & -42.658920 & 512 $\pm$ 29 & p & 20.64 & 20.22 & 1 \\
H20-1605 & GC0410 & AAT222977;T17-2118 & 201.74551 & -42.648139 & 655 $\pm$ 112 & m & 20.17 & 19.89 & 1 \\
H20-1612 & GC0387 & AAT215171;T17-1995 & 201.58615 & -42.642176 & 527 $\pm$ 48 & m & 19.60 & 19.10 & 1 \\
H20-1690 & HHH86-16 & GC0244;HHH86-16;T17-1639 & 201.39590 & -42.601351 & 552 $\pm$ 37 & m & 18.51 & 17.99 & 1 \\
H20-1725 & pff\_gc-096 & PFF096;GC0402;PFF-gc096;T17-2038 & 201.62623 & -42.578209 & 483 $\pm$ 122 & m & 19.73 & 19.17 & 1 \\
H20-1778 & pff\_gc-080 & PFF080;GC0343;PFF-gc080;T17-1868 & 201.49817 & -42.544245 & 616 $\pm$ 123 & m & 19.80 & 19.39 & 1 \\
H20-1800 & pff\_gc-077 & PFF077;GC0338;T17-1860 & 201.49236 & -42.527250 & 675 $\pm$ 41 & l & 19.33 & 18.96 & 1 \\
H20-1818 & GC0323 & AAT209412;T17-1809 & 201.47210 & -42.514613 & 998 $\pm$ 250 & m & 20.21 & 19.64 & 1 \\
H20-1893 & GC0549 & T17-2032 & 201.62045 & -43.223498 & 459 $\pm$ 31 & p & 21.20 & 20.41 & 1 \\
H20-1918 & N32 & GC0556;T17-2092 & 201.69158 & -43.194909 & 563 $\pm$ 39 & p & 20.31 & 19.83 & 1 \\
H20-1923 &           86 & WHH-31;GC0405;GC0405;T17-2073 & 201.67268 & -43.190278 & 572 $\pm$ 67 & p & 19.64 & 18.92 & 1 \\
H20-2022 & GC605 & GC0605;T17-2108 & 201.72528 & -43.085036 & 948 $\pm$ 64 & p & 19.52 & 18.95 & 1 \\
H20-2055 & GC551 & GC0551;T17-2040 & 201.62688 & -43.054253 & 349 $\pm$ 91 & p & 20.63 & 20.08 & 1 \\
H20-2123 & GC0559 & T17-2130 & 201.76193 & -42.984643 & 278 $\pm$ 29 & p & 19.50 & 18.94 & 1 \\
H20-2671 & pff\_gc-097 & PFF097;GC0407;PFF-gc097;T17-2091 & 201.68908 & -43.442803 & 642 $\pm$ 47 & m & 18.62 & 18.02 & 1 \\
H20-2841 & GC0558 & T17-2114 & 201.73264 & -43.336506 & 616 $\pm$ 25 & p & 19.33 & 18.69 & 1 \\
H20-2867 & pff\_gc-098 & GC0409;PFF-gc098;GC0409;T17-2107 & 201.72469 & -43.321572 & 605 $\pm$ 12 & p & 18.25 & 17.52 & 1 \\
H20-2878 & GC0555 & T17-2086 & 201.68477 & -43.319598 & 336 $\pm$ 33 & p & 19.93 & 19.35 & 1 \\
H20-2931 & N30 & GC0554;T17-2080 & 201.67579 & -43.286636 & 415 $\pm$ 36 & p & 20.11 & 19.56 & 1 \\
H20-3074 & pff\_gc-013 & GC0042;PFF-gc013;T17-1203 & 201.16836 & -43.584691 & 839 $\pm$ 63 & m & 18.88 & 18.20 & 1 \\
H20-3107 & GC0352 & AAT329848;T17-1887 & 201.50529 & -43.570986 & 558 $\pm$ 46 & m & 18.31 & 17.63 & 1 \\
H20-3488 & GC0190 & AAT321194;T17-1531 & 201.33883 & -43.399800 & 254 $\pm$ 169 & m & 20.04 & 19.32 & 1 \\
H20-3544 & GC0547 & T17-2009 & 201.59615 & -43.377542 & 521 $\pm$ 57 & p & 21.21 & 20.43 & 1 \\
H20-3550 & GC0522 & T17-1589 & 201.37541 & -43.375909 & 573 $\pm$ 48 & p & 20.97 & 20.25 & 1 \\
H20-3554 & GC0513 & T17-1524 & 201.33379 & -43.372707 & 844 $\pm$ 54 & p & 20.67 & 20.10 & 1 \\
H20-3577 & pff\_gc-008 & PFF008;GC0029;PFF-gc008;T17-1161 & 201.12165 & -43.365677 & 520 $\pm$ 80 & m & 19.90 & 19.15 & 1 \\
H20-3591 & GC0025 & AAT308432;T17-1145 & 201.10646 & -43.359846 & 835 $\pm$ 83 & m & 19.36 & 18.56 & 1 \\
H20-3601 & HGHH-34 & C34;GC0270;HGHH-34;GC0270;T17-1688 & 201.41916 & -43.353833 & 631 $\pm$ 9 & p & 18.40 & 17.62 & 1 \\
H20-3620 & pff\_gc-024 & PFF024;GC0081;PFF-gc024;GC0081;T17-1297 & 201.23207 & -43.344198 & 279 $\pm$ 38 & p & 19.77 & 19.13 & 1 \\
H20-3632 & C41 & C41;HGHH-41;HGHH92-C41;GC0040;HGHH-41;GC0040;0040;T17-1197 & 201.16239 & -43.335105 & 363 $\pm$ 1 & p & 18.58 & 17.82 & 1 \\
H20-3648 & pff\_gc-076 & PFF076;pff\_gc-076;GC0327;PFF-gc076;GC0327;T17-1815 & 201.47393 & -43.330166 & 335 $\pm$ 6 & p & 19.09 & 18.15 & 1 \\
H20-3662 & HGHH-44 & C44;C44;HGHH-44;C44;C44;HGHH92-C44;GC0227;HGHH-44;GC0227;0227;T17-1611 & 201.38224 & -43.322960 & 505 $\pm$ 1 & p & 18.58 & 17.93 & 1 \\
H20-3666 & pff\_gc-011 & PFF011;PFF011;GC0037;PFF-gc011;GC0037;T17-1188 & 201.15359 & -43.321160 & 570 $\pm$ 31 & p & 18.89 & 18.33 & 1 \\
H20-3684 & C112 & GC0034;T17-1177 & 201.13613 & -43.313556 &   &    & 21.70 & 21.06 &   \\
H20-3696 & GC0494 & T17-1323 & 201.24292 & -43.309329 & 676 $\pm$ 42 & p & 20.48 & 19.95 & 1 \\
H20-3699 & GC0571 & T17-1189 & 201.15402 & -43.308833 & 926 $\pm$ 44 & p & 20.41 & 19.66 & 1 \\
H20-3702 & GC0546 & T17-2001 & 201.59055 & -43.307999 & 507 $\pm$ 84 & p & 21.30 & 20.68 & 1 \\
H20-3713 & C29 & C29;HGHH-29;C29;C29;HGHH92-C29;GC0041;HGHH-29;GC0041;0041;T17-1202 & 201.16827 & -43.301452 & 725 $\pm$ 1 & p & 18.11 & 17.22 & 1 \\
H20-3746 & C111 & GC0026;T17-1153 & 201.11239 & -43.288872 &   &    & 21.45 & 20.99 &   \\
H20-3748 & GC0423 & T17-1382 & 201.26785 & -43.286355 & 524 $\pm$ 41 & p & 21.08 & 20.49 & 1 \\
H20-3766 & GC0428 & T17-1535 & 201.34235 & -43.277468 & 417 $\pm$ 47 & p & 20.05 & 19.50 & 1 \\
H20-3769 & pff\_gc-044 & PFF044;pff\_gc-042;GC0151;GC0151;T17-1458 & 201.30492 & -43.276530 & 568 $\pm$ 53 & p & 19.22 & 18.67 & 1 \\
H20-3770 & pff\_gc-042 & PFF042;GC0146;PFF-gc042;GC0146;T17-1447 & 201.30082 & -43.276057 & 573 $\pm$ 16 & p & 18.84 & 18.27 & 1 \\
H20-3773 & C113 & GC0038;GC0038;T17-1191 & 201.15733 & -43.274018 & 212 $\pm$ 10 & p & 19.45 & 18.89 &   \\
H20-3789 & GC0600 & T17-1961 & 201.54879 & -43.268189 & 355 $\pm$ 40 & p & 19.49 & 18.76 & 1 \\
H20-3811 & pff\_gc-043 & PFF043;GC0148;PFF-gc043;GC0148;T17-1449 & 201.30182 & -43.235389 & 526 $\pm$ 33 & p & 19.31 & 18.68 & 1 \\
H20-3817 & pff\_gc-036 & PFF036;GC0122;PFF-gc036;GC0122;T17-1393 & 201.27268 & -43.234055 & 679 $\pm$ 13 & p & 18.91 & 18.30 & 1 \\
H20-3840 & pff\_gc-051 & PFF051;GC0192;PFF-gc051;GC0192;T17-1538 & 201.34307 & -43.250044 & 451 $\pm$ 30 & p & 19.78 & 19.05 & 1 \\
H20-3856 & HHH86-13 & C13;C13;GC0125;HHH86-13;GC0125;T17-1400 & 201.27595 & -43.253218 & 597 $\pm$ 10 & p & 18.63 & 17.91 & 1 \\
H20-3874 & pff\_gc-033 & PFF033;GC0112;T17-1373 & 201.26386 & -43.257613 & 531 $\pm$ 18 & l & 19.51 & 18.73 & 1 \\
H20-3878 & GC0517 & T17-1552 & 201.35316 & -43.227053 & 798 $\pm$ 60 & p & 20.41 & 19.80 & 1 \\
H20-3892 &           51 & WHH-4;GC0044;HH-024;GC0044;T17-1206 & 201.16916 & -43.221638 & 699 $\pm$ 17 & p & 19.10 & 18.23 & 1 \\
H20-4059 & pff\_gc-003 & PFF003;GC0014;PFF-gc003;T17-1060 & 201.01348 & -43.470498 & 771 $\pm$ 69 & m & 19.33 & 18.72 & 1 \\
H20-4211 & GC0483 & T17-1086 & 201.04115 & -43.377495 & 756 $\pm$ 37 & p & 21.42 & 20.64 & 1 \\
H20-4233 & GC0481 & T17-1034 & 200.97577 & -43.365720 & 512 $\pm$ 84 & p & 22.19 & 21.32 & 1 \\
H20-4357 & pff\_gc-002 & PFF002;GC0011;PFF-gc002;GC0011;T17-1053 & 200.99793 & -43.291394 & 652 $\pm$ 37 & p & 19.50 & 18.89 & 1 \\
H20-4363 & GC0482 & T17-1063 & 201.01664 & -43.288983 & 599 $\pm$ 105 & p & 22.16 & 21.52 & 1 \\
H20-4467 & pff\_gc-001 & PFF001;GC0006;PFF-gc001;T17-1020 & 200.95672 & -43.242202 & 702 $\pm$ 47 & m & 18.92 & 18.23 & 1 \\
H20-4470 & pff\_gc-005 & PFF005;GC0020;PFF-gc005;GC0020;T17-1112 & 201.07881 & -43.241713 & 749 $\pm$ 32 & p & 20.33 & 19.59 & 1 \\
H20-6992 & pff\_gc-100 & GC0413;PFF-gc100;T17-2133 & 201.76423 & -42.454746 & 527 $\pm$ 31 & m & 18.50 & 17.82 & 1 \\
H20-7126 & pff\_gc-082 & PFF082;GC0349;PFF-gc082;T17-1881 & 201.50405 & -42.367630 & 593 $\pm$ 42 & m & 19.27 & 18.56 & 1 \\
H20-9080 & pff\_gc-102 & PFF102;GC0415;PFF-gc102;T17-2317 & 202.07694 & -42.553438 & 576 $\pm$ 119 & m & 19.33 & 18.79 & 1 \\
H20-11286 & R209 & GC0257;R209;GC0257;0257;T17-1666 & 201.40888 & -43.217307 & 558 $\pm$ 43 & p & 20.63 & 20.02 & 1 \\
H20-11287 &          192 & N11;GC0489;T17-1211 & 201.17296 & -43.214762 & 506 $\pm$ 41 & p & 20.68 & 20.19 & 1 \\
H20-11298 & pff\_gc-037 & f2.GC-74;GC0128;GC0128;0128;T17-1409 & 201.28117 & -43.208196 & 548 $\pm$ 21 & p & 20.41 & 19.86 & 1 \\
H20-11302 & GC0492 & T17-1307 & 201.23593 & -43.206538 & 713 $\pm$ 28 & p & 20.91 & 20.49 & 1 \\
H20-11306 & C2 & C2;VHH81-02;C2;C2;GC0067;VHH81-02;GC0067;T17-1264 & 201.21451 & -43.203093 & 624 $\pm$ 13 & p & 18.39 & 17.84 & 1 \\
H20-11310 & N12 & GC0416;T17-1181 & 201.14013 & -43.200433 & 546 $\pm$ 9 & p & 20.57 & 20.04 & 1 \\
H20-11317 & HHH86-15 & C15;C15;HHH86-C15=R226;GC0218;HHH86-15;GC0218;0218;T17-1596 & 201.37669 & -43.197127 & 663 $\pm$ 1 & p & 18.60 & 17.91 & 1 \\
H20-11323 & R229 & GC0212;0212;T17-1585 & 201.37392 & -43.195240 & 517 $\pm$ 66 & l & 19.64 & 19.13 & 1 \\
H20-11325 & pff\_gc-034 & PFF034;PFF034;GC0114;T17-1376 & 201.26401 & -43.194362 & 605 $\pm$ 46 & l & 19.84 & 19.33 & 1 \\
H20-11326 & pff\_gc-067 & PFF067;GC0304;PFF-gc067;GC0304;T17-1765 & 201.45323 & -43.194115 & 631 $\pm$ 42 & p & 19.56 & 19.09 & 1 \\
H20-11327 & GC0491 & T17-1290 & 201.22911 & -43.193578 & 670 $\pm$ 19 & p & 20.97 & 20.25 & 1 \\
H20-11332 & GC0495 & T17-1330 & 201.24569 & -43.191146 & 508 $\pm$ 15 & p & 20.68 & 19.96 & 1 \\
H20-11333 & pff\_gc-009 & PFF009;N10;GC0032;PFF-gc009;GC0032;T17-1171 & 201.13054 & -43.190781 & 734 $\pm$ 25 & p & 19.67 & 19.16 & 1 \\
H20-11337 & pff\_gc-031 & PFF031;PFF031;GC0108;GC0108;0108;T17-1365 & 201.26145 & -43.189257 & 456 $\pm$ 26 & p & 19.40 & 18.89 & 1 \\
H20-11343 & C125 & GC0099;GC0099;T17-1344 & 201.25347 & -43.186280 & 941 $\pm$ 66 & p & 21.09 & 20.55 & 1 \\
H20-11351 &           81 & WHH-3;GC0033;WHH-03;GC0033;T17-1176 & 201.13401 & -43.182469 & 775 $\pm$ 32 & p & 19.41 & 18.89 & 1 \\
H20-11359 & GC0059 & AAT110138;GC0059;T17-1239 & 201.19829 & -43.180150 & 344 $\pm$ 37 & p & 19.62 & 19.06 & 1 \\
H20-11360 & pff\_gc-035 & PFF035;PFF035;GC0117;PFF-gc035;GC0117;0117;T17-1384 & 201.26859 & -43.180141 & 626 $\pm$ 22 & p & 19.79 & 19.09 & 1 \\
H20-11362 & C124 & GC0097;T17-1342 & 201.25158 & -43.179711 &   &    & 21.97 & 21.62 &   \\
H20-11364 & f2.GC-63 & GC0506;T17-1451 & 201.30322 & -43.178745 & 280 $\pm$ 29 & p & 20.93 & 20.22 & 1 \\
H20-11366 & R202 & GC0275;R202;GC275;T17-1703 & 201.42497 & -43.178275 & 279 $\pm$ 60 & m & 19.36 & 18.85 & 1 \\
H20-11368 & GC0419 & T17-1293 & 201.23050 & -43.177568 & 656 $\pm$ 27 & p & 20.56 & 19.83 & 1 \\
H20-11370 & pff\_gc-089 & C49;pff\_gc-089;GC0385;PFF-gc089;GC385;T17-1990 & 201.58421 & -43.176569 & 548 $\pm$ 36 & m & 18.88 & 18.39 & 1 \\
H20-11375 & HGHH-12 & HGHH-12;C12;C12;HGHH92-C12=R281;GC0123;GC0123;0123;T17-1395 & 201.27375 & -43.175226 & 439 $\pm$ 1 & p & 17.99 & 17.29 & 1 \\
H20-11385 & AAT111563 & GC0083;AAT111563;GC083;GC0083;0083;T17-1301 & 201.23364 & -43.171200 & 687 $\pm$ 31 & p & 20.21 & 19.92 & 1 \\
H20-11389 & GC533 & GC0533;T17-1830 & 201.47961 & -43.167986 & 354 $\pm$ 25 & p & 20.64 & 20.03 & 1 \\
H20-11394 & f2.GC-69 & f2.GC69;GC584;GC0584;T17-1421 & 201.28780 & -43.167212 & 552 $\pm$ 26 & p & 19.95 & 19.34 & 1 \\
H20-11395 & GC490 & GC0490;T17-1236 & 201.19752 & -43.166604 & 568 $\pm$ 22 & p & 20.88 & 20.18 & 1 \\
H20-11397 & N25 & GC544;GC0544;T17-1980 & 201.57203 & -43.166085 & 473 $\pm$ 39 & p & 21.59 & 20.77 & 1 \\
H20-11400 & R235 & f2.GC-35;GC0204;R235;GC204;GC0204;0204;T17-1567 & 201.36175 & -43.161253 & 524 $\pm$ 23 & p & 19.47 & 19.02 & 1 \\
H20-11401 & GC0347 & K-217;GC347;T17-1879 & 201.50336 & -43.161123 & 314 $\pm$ 157 & m & 20.20 & 19.53 & 1 \\
H20-11403 & HGHH-43 & HGHH-43;C43;C43;GC0119;HGHH-43;GC119;GC0119;T17-1386 & 201.26999 & -43.160792 & 481 $\pm$ 10 & p & 18.58 & 18.04 & 1 \\
H20-11409 & R254 & GC0174;R254;GC174;GC0174;T17-1496 & 201.32061 & -43.157780 & 561 $\pm$ 26 & p & 19.40 & 18.86 & 1 \\
H20-11410 & HGHH-4 & HGHH-04;C4;C4;C4;GC0106;HGHH-04;GC106;0106;T17-1358 & 201.25756 & -43.157065 & 724 $\pm$ 46 & m & 17.95 & 17.44 & 1 \\
H20-11418 & f2.GC-21 & GC523;GC0523;T17-1619 & 201.38797 & -43.156000 & 351 $\pm$ 69 & p & 20.81 & 20.35 & 1 \\
H20-11430 & GC0362 & AAT122808;GC362;GC0362;T17-1913 & 201.51920 & -43.152831 & 264 $\pm$ 131 & p & 20.07 & 19.63 & 1 \\
H20-11431 &           41 & WHH-27;GC0379;GC379;T17-1968 & 201.55347 & -43.152548 & 545 $\pm$ 60 & l & 18.75 & 18.05 & 1 \\
H20-11433 & R271 & C132;GC0131;GC131;0131;T17-1418 & 201.28666 & -43.152657 & 436 $\pm$ 45 & l & 19.36 & 18.87 & 1 \\
H20-11434 & C123 & GC0095;GC095;GC0095;0095;T17-1337 & 201.24970 & -43.152380 & 374 $\pm$ 34 & p & 20.74 & 20.22 & 1 \\
H20-11440 & GC502 & GC0502;T17-1401 & 201.27782 & -43.149512 & 240 $\pm$ 53 & p & 21.45 & 20.67 &   \\
H20-11442 & pff\_gc-084 & PFF084;GC0354;PFF-gc084;GC354;GC0354;0354;T17-1895 & 201.50938 & -43.148794 & 457 $\pm$ 38 & p & 19.88 & 19.20 & 1 \\
H20-11446 & f2.GC-70 & f2.GC70;GC504;GC0504;T17-1420 & 201.28725 & -43.148238 & 678 $\pm$ 26 & p & 20.22 & 19.85 & 1 \\
H20-11448 & f2.GC-36 & GC0202;AAT116531;0202;T17-1565 & 201.36150 & -43.148155 & 267 $\pm$ 71 & m & 19.72 & 19.21 & 1 \\
H20-11449 & GC598 & GC0598;T17-1950 & 201.53974 & -43.147886 & 483 $\pm$ 67 & p & 20.09 & 19.40 & 1 \\
H20-11455 & C127 & GC0101;T17-1350 & 201.25551 & -43.145370 &   &    & 21.93 & 21.37 &   \\
H20-11456 & C118 & GC0085;GC085;T17-1312 & 201.23832 & -43.145195 &   &    & 21.41 & 20.74 &   \\
H20-11458 & R257 & GC0162;GC162;0162;T17-1477 & 201.31346 & -43.144221 & 339 $\pm$ 51 & l & 20.90 & 20.22 & 1 \\
H20-11459 & R253 & GC0177;R253;GC0177;T17-1499 & 201.32217 & -43.144162 & 485 $\pm$ 52 & p & 19.64 & 19.11 & 1 \\
H20-11460 & GC0030 & AAT107060;T17-1162 & 201.12173 & -43.143498 & 600 $\pm$ 58 & m & 20.35 & 19.66 & 1 \\
H20-11461 & R215 & GC0250;R215;GC250;GC0250;0250;T17-1650 & 201.39851 & -43.143574 & 542 $\pm$ 56 & p & 20.79 & 20.19 & 1 \\
H20-11464 & C128 & GC0102;GC102;T17-1352 & 201.25613 & -43.142494 &   &    & 21.58 & 20.83 &   \\
H20-11467 &           64 & WHH-28;GC0380;GC380;T17-1970 & 201.55917 & -43.141774 & 506 $\pm$ 123 & l & 19.15 & 18.63 & 1 \\
H20-11468 & R276 & GC0126;GC126;GC0126;0126;T17-1407 & 201.28052 & -43.141559 & 550 $\pm$ 28 & p & 20.74 & 20.19 & 1 \\
H20-11473 & GC0292 & AAT119596;AAT119596;GC0292;T17-1740 & 201.44188 & -43.140131 & 595 $\pm$ 14 & p & 19.78 & 19.09 & 1 \\
H20-11479 &          148 & GC0063;AAT110410;GC063;GC0063;T17-1255 & 201.20571 & -43.138235 & 567 $\pm$ 76 & p & 20.28 & 19.73 & 1 \\
H20-11481 & R203 & f2.GC03;GC0272;R203;GC272;R203;GC0272;T17-1693 & 201.42045 & -43.137773 & 446 $\pm$ 31 & p & 19.74 & 19.31 & 1 \\
H20-11482 & HHH86-10 & C10;C10;GC0060;HHH86-10;GC060;GC0060;T17-1243 & 201.20016 & -43.137276 & 786 $\pm$ 18 & p & 18.46 & 17.84 & 1 \\
H20-11488 & pff\_gc-065 & PFF065;GC0297;GC297;GC0297;T17-1750 & 201.44549 & -43.135177 & 417 $\pm$ 12 & p & 19.27 & 18.64 & 1 \\
H20-11489 & pff\_gc-078 & PFF078;GC0339;PFF-gc078;GC339;T17-1861 & 201.49363 & -43.135077 & 546 $\pm$ 42 & m & 19.41 & 18.69 & 1 \\
H20-11491 & C155 & GC0253;GC253;T17-1656 & 201.40204 & -43.134267 &   &    & 21.65 & 21.14 &   \\
H20-11492 & GC529 & GC0529;T17-1788 & 201.46063 & -43.134117 & 720 $\pm$ 80 & p & 20.56 & 20.17 & 1 \\
H20-11496 & R261 & R261;GC0150;R261;GC150;R261;GC0150;0150;T17-1455 & 201.30369 & -43.133100 & 616 $\pm$ 3 & p & 18.26 & 17.62 & 1 \\
H20-11497 & f2.GC-40 & GC0195;AAT116220;GC195;GC0195;0195;T17-1551 & 201.35165 & -43.133013 & 542 $\pm$ 34 & p & 19.51 & 18.91 & 1 \\
H20-11501 & pff\_gc-063 & PFF063;PFF063;GC0284;GC284;GC0284;T17-1721 & 201.43251 & -43.131921 & 534 $\pm$ 58 & p & 19.72 & 19.31 & 1 \\
H20-11504 & GC0371 & AAT123188;GC371;0371;T17-1934 & 201.52888 & -43.131284 & 364 $\pm$ 56 & m & 20.44 & 19.82 & 1 \\
H20-11508 & R247 & GC0186;GC186;R247;T17-1522 & 201.33315 & -43.128834 & 723 $\pm$ 33 & o & 20.23 & 19.53 & 1 \\
H20-11513 &          163 & GC0064;AAT110551;GC064;GC0064;0064;T17-1257 & 201.20865 & -43.126716 & 594 $\pm$ 36 & p & 20.30 & 20.00 & 1 \\
H20-11514 & R259 & GC0154;GC154;R259;GC0154;0154;T17-1463 & 201.30778 & -43.125703 & 623 $\pm$ 29 & p & 20.80 & 20.22 & 1 \\
H20-11518 & HGHH-19 & C19;C19;C19;GC0282;HGHH-19;C19;GC0282;T17-1719 & 201.43083 & -43.123013 & 613 $\pm$ 6 & p & 18.11 & 17.53 & 1 \\
H20-11519 &           78 & WHH-11;GC0158;K-051;GC158;WHH-11;GC0158;T17-1470 & 201.30937 & -43.123203 & 616 $\pm$ 18 & p & 19.63 & 18.87 & 1 \\
H20-11522 & R204 & C161;GC0269;GC0269;0269;T17-1686 & 201.41891 & -43.121607 & 443 $\pm$ 23 & p & 19.84 & 19.14 & 1 \\
H20-11523 & R224 & C149;GC0229;GC229;GC0229;0229;T17-1613 & 201.38474 & -43.121402 & 456 $\pm$ 20 & p & 20.06 & 19.61 & 1 \\
H20-11527 & HGHH-G143 & HGHH-G143;G143;GC0340;HGHH-G143;GC340;G143;GC0340;T17-1863 & 201.49451 & -43.119727 & 500 $\pm$ 19 & p & 19.16 & 18.63 & 1 \\
H20-11530 & GC597 & GC0597;T17-1930 & 201.52737 & -43.118927 & 240 $\pm$ 30 & p & 20.54 & 19.89 &   \\
H20-11533 &          126 & GC0375;AAT123656;GC375;T17-1951 & 201.54001 & -43.118335 & 380 $\pm$ 93 & m & 20.12 & 19.39 & 1 \\
H20-11534 &          174 & GC493;GC0493;T17-1319 & 201.24124 & -43.118419 & 559 $\pm$ 40 & p & 20.63 & 19.96 & 1 \\
H20-11539 & R223 & f2.GC23;R223;GC0232;R223;GC232;R223;0232;T17-1616 & 201.38667 & -43.117283 & 766 $\pm$ 23 & o & 18.80 & 18.19 & 1 \\
H20-11542 & GC0350 & AAT122146;GC350;GC0350;0350;T17-1882 & 201.50414 & -43.115358 & 517 $\pm$ 99 & p & 20.04 & 19.48 & 1 \\
H20-11543 & f2.GC-28 & f2.GC28;GC465;GC0465;T17-1591 & 201.37577 & -43.115142 & 642 $\pm$ 58 & o & 21.54 & 20.92 &   \\
H20-11549 & C167 & GC0290;GC290;T17-1737 & 201.44153 & -43.112607 &   &    & 20.76 & 20.23 &   \\
H20-11551 &          209 & GC421;GC0421;0421;T17-1335 & 201.24826 & -43.111332 & 726 $\pm$ 30 & p & 21.13 & 20.36 & 1 \\
H20-11553 & f2.GC-46 & GC0188;AAT115679;GC188;AAT115679;GC0188;0188;T17-1529 & 201.33627 & -43.109967 & 817 $\pm$ 47 & p & 20.71 & 19.87 &   \\
H20-11555 &          154 & GC418;GC0418;0418;T17-1224 & 201.18658 & -43.109231 & 374 $\pm$ 30 & p & 20.26 & 19.52 & 1 \\
H20-11557 & GC572 & GC0572;T17-1190 & 201.15564 & -43.108690 & 183 $\pm$ 49 & p & 20.77 & 20.09 &   \\
H20-11560 & pff\_gc-012 & PFF012;GC0039;GC039;T17-1196 & 201.16148 & -43.107393 & 573 $\pm$ 21 & l & 19.57 & 18.84 & 1 \\
H20-11567 & GC0515 & T17-1543 & 201.34619 & -43.105794 & 591 $\pm$ 29 & p & 21.06 & 20.38 &   \\
H20-11568 & GC0127 & AAT113428;GC127;AAT113428;0127;T17-1406 & 201.28050 & -43.105715 & 700 $\pm$ 36 & o & 20.05 & 19.44 & 1 \\
H20-11574 & pff\_gc-086 & PFF086;GC0368;PFF-gc086;GC368;GC0368;T17-1928 & 201.52728 & -43.104029 & 439 $\pm$ 25 & p & 20.03 & 19.36 & 1 \\
H20-11576 & GC460 & GC0460;GC0460;T17-1526 & 201.33510 & -43.102495 & 737 $\pm$ 17 & p & 20.51 & 19.79 &   \\
H20-11577 & pff\_gc-066 & PFF066;PFF066;GC0299;PFF-gc066;GC299;pff\_gc-066;0299;T17-1754 & 201.44643 & -43.102454 & 515 $\pm$ 28 & o & 19.93 & 19.34 & 1 \\
H20-11578 & AAT120336 & GC0311;AAT120336;GC311;T17-1783 & 201.45923 & -43.102364 & 452 $\pm$ 67 & m & 20.24 & 19.57 & 1 \\
H20-11582 & pff\_gc-018 & PFF018;pff\_gc-018;GC0056;PFF-gc018;GC056;pff\_gc-018;GC0056;T17-1233 & 201.19617 & -43.100463 & 528 $\pm$ 12 & p & 19.06 & 18.27 & 1 \\
H20-11592 & C21 & C21;HGHH-21;C21;C21;HGHH92-C21;GC0320;HGHH-21;GC320;GC0320;0320;T17-1805 & 201.46975 & -43.096230 & 461 $\pm$ 1 & p & 17.82 & 17.25 & 1 \\
H20-11597 &          185 & C148;GC0228;GC228;0228;T17-1612 & 201.38234 & -43.096078 &   &    & 20.12 & 19.91 &   \\
H20-11599 & AAT118198 & GC0255;AAT118198;GC255;AAT118198;T17-1662 & 201.40611 & -43.095800 & 524 $\pm$ 18 & o & 19.77 & 19.02 &   \\
H20-11602 & GC0358 & AAT122526;GC358;0358;T17-1900 & 201.51204 & -43.095261 & 506 $\pm$ 50 & m & 20.44 & 19.71 & 1 \\
H20-11603 & GC0466 & T17-1595 & 201.37642 & -43.095198 & 379 $\pm$ 50 & o & 20.60 & 20.10 &   \\
H20-11609 & GC0075 & AAT111296;GC075;GC0075;0075;T17-1285 & 201.22698 & -43.092967 & 695 $\pm$ 45 & p & 20.08 & 19.34 & 1 \\
H20-11610 & C158 & GC0261;GC261;0261;T17-1674 & 201.41159 & -43.092896 &   &    & 20.44 & 19.85 &   \\
H20-11611 & pff\_gc-025 & PFF025;GC0088;GC088;pff\_gc-025;T17-1315 & 201.23976 & -43.092440 & 864 $\pm$ 30 & o & 20.04 & 19.35 & 1 \\
H20-11619 & pff\_gc-052 & PFF052;PFF052;GC0199;GC199;pff\_gc-052;GC0199;0199;T17-1558 & 201.35726 & -43.087922 & 534 $\pm$ 31 & p & 19.85 & 19.34 &   \\
H20-11620 &          137 & GC595;GC0595;T17-1855 & 201.49054 & -43.087009 & 410 $\pm$ 37 & p & 20.09 & 19.33 & 1 \\
H20-11623 &          157 & C146;GC0214;GC214;0214;T17-1587 & 201.37451 & -43.085879 &   &    & 20.45 & 19.86 &   \\
H20-11624 & pff\_gc-049 & PFF049;GC0165;GC165;pff\_gc-049;GC0165;0165;T17-1481 & 201.31692 & -43.085123 & 707 $\pm$ 19 & p & 19.60 & 19.03 &   \\
H20-11627 & GC0307 & AAT120259;GC307;GC0307;T17-1775 & 201.45717 & -43.084635 & 477 $\pm$ 54 & p & 20.23 & 19.50 & 1 \\
H20-11628 & HHH86-18 & C18;C18;C18/K163;HHH86-C18;GC0266;HHH86-18;GC266;C18;T17-1683 & 201.41615 & -43.083822 & 442 $\pm$ 7 & o & 17.49 & 16.96 &   \\
H20-11631 &          238 & C162;GC0271;GC271;T17-1691 & 201.42033 & -43.083434 &   &    & 20.76 & 20.44 &   \\
H20-11634 & C165 & GC0283;GC283;GC0283;T17-1720 & 201.43102 & -43.082333 & 316 $\pm$ 14 & p & 18.81 & 18.12 &   \\
H20-11638 & GC446 & GC0446;GC0446;T17-1258 & 201.21027 & -43.080846 & 370 $\pm$ 20 & p & 19.89 & 19.10 & 1 \\
H20-11641 & GC426 & LDSS2-30585;GC0426;0426;T17-1469 & 201.30913 & -43.079622 & 858 $\pm$ 30 & p & 20.24 & 19.79 &   \\
H20-11644 & GC543 & GC0543;T17-1945 & 201.53557 & -43.079158 & 466 $\pm$ 33 & p & 20.70 & 20.19 & 1 \\
H20-11646 & GC0475 & T17-1743 & 201.44309 & -43.078893 & 550 $\pm$ 55 & o & 20.68 & 20.02 &   \\
H20-11648 &          194 & GC0601;T17-1969 & 201.55551 & -43.077994 & 184 $\pm$ 43 & p & 20.73 & 19.99 &   \\
H20-11652 & C144 & GC0201;T17-1563 & 201.35959 & -43.077367 &   &    & 21.86 & 21.11 &   \\
H20-11654 & GC425 & LDSS2-34333;GC0425;0425;T17-1427 & 201.29003 & -43.077197 & 648 $\pm$ 19 & p & 20.48 & 20.00 &   \\
H20-11657 & C159 & GC0262;GC262;GC0262;0262;T17-1676 & 201.41329 & -43.076043 & 354 $\pm$ 140 & p & 20.67 & 19.96 &   \\
H20-11664 & C166 & GC0287;T17-1727 & 201.43709 & -43.072484 &   &    & 21.79 & 21.02 &   \\
H20-11665 & HGHH-G327 & HGHH-G327;G327;GC0144;HGHH-G327;GC144;GC0144;0144;T17-1443 & 201.29984 & -43.072016 & 622 $\pm$ 18 & p & 19.92 & 19.20 &   \\
H20-11667 & AAT117287 & GC0223;AAT117287;GC0223;T17-1605 & 201.37947 & -43.071361 & 554 $\pm$ 60 & p & 20.54 & 19.76 &   \\
H20-11668 & pff\_gc-038 & PFF038;GC0132;GC132;pff\_gc-038;T17-1417 & 201.28672 & -43.070798 & 436 $\pm$ 16 & o & 19.38 & 18.69 &   \\
H20-11672 & HGHH-G19 & G19;HGHH-G019;G019;GC0054;HGHH-G019;GC054;GC0054;0054;T17-1230 & 201.19352 & -43.069882 & 712 $\pm$ 20 & p & 19.06 & 18.57 & 1 \\
H20-11673 & AAT115339 & GC0181;AAT115339;GC181;GC0181;0181;T17-1509 & 201.32682 & -43.069391 & 618 $\pm$ 108 & p & 20.05 & 19.48 &   \\
H20-11675 &          124 & WHH-25;GC0312;WHH-25;GC312;WHH-25;GC0312;0312;T17-1784 & 201.45984 & -43.068963 & 468 $\pm$ 36 & p & 20.02 & 19.39 &   \\
H20-11677 &           57 & WHH-16;WHH16/K102;GC0205;K-102;GC205;WHH-16;GC0205;T17-1571 & 201.36661 & -43.067259 & 715 $\pm$ 10 & p & 19.27 & 18.55 &   \\
H20-11683 & pff\_gc-075 & PFF075;pff\_gc-075;GC0325;PFF-gc075;GC325;pff\_gc-075;GC0325;T17-1813 & 201.47288 & -43.065726 & 728 $\pm$ 13 & p & 19.52 & 18.87 & 1 \\
H20-11686 & C151 & GC0236;GC236;GC0236;0236;T17-1624 & 201.39142 & -43.064266 & 299 $\pm$ 67 & p & 20.91 & 19.99 &   \\
H20-11687 & C147 & GC0219;GC219;0219;T17-1597 & 201.37779 & -43.063113 &   &    & 20.34 & 19.81 &   \\
H20-11689 & C163 & GC0274;GC274;GC0274;0274;T17-1699 & 201.42349 & -43.062715 & 701 $\pm$ 43 & p & 20.74 & 20.15 &   \\
H20-11691 & GC461 & GC0461;T17-1548 & 201.34997 & -43.062557 & 527 $\pm$ 74 & o & 20.79 & 20.28 &   \\
H20-11694 &           79 & WHH-30;GC0395;GC395;GC0395;T17-2011 & 201.59840 & -43.062175 & 470 $\pm$ 66 & p & 19.38 & 18.80 & 1 \\
H20-11696 &          153 & AAT119508;GC0279;AAT119058;GC279;AAT119058;T17-1712 & 201.42717 & -43.061509 & 385 $\pm$ 87 & m & 20.57 & 19.80 &   \\
H20-11700 & C136 & GC0157;T17-1468 & 201.30869 & -43.059715 &   &    & 21.35 & 20.80 &   \\
H20-11701 & C154 & GC0243;C154;T17-1636 & 201.39463 & -43.058354 & 719 $\pm$ 86 & o & 20.05 & 19.43 &   \\
H20-11702 &          315 & C157;GC0259;GC259;GC0259;T17-1669 & 201.41023 & -43.057978 & 574 $\pm$ 106 & p & 19.34 & 18.90 &   \\
H20-11705 & HCH21 &          310;C153;GC0242;HCH21;GC0242;0242;T17-1635 & 201.39437 & -43.057693 & 662 $\pm$ 1 & p & 18.76 & 18.16 &   \\
H20-11713 & C140 & GC0178;T17-1501 & 201.32267 & -43.056996 &   &    & 20.29 & 19.70 &   \\
H20-11714 & AAT113992 & GC0140;AAT113992;GC140;0140;T17-1433 & 201.29374 & -43.056667 & 648 $\pm$ 58 & m & 20.45 & 19.78 &   \\
H20-11719 & C50 & C50;GC0384;K-233;GC384;GC0384;0384;T17-1989 & 201.58192 & -43.055162 & 690 $\pm$ 22 & p & 18.76 & 18.12 & 1 \\
H20-11720 & C164 & GC0276;GC276;GC0276;T17-1705 & 201.42537 & -43.055381 & 536 $\pm$ 25 & p & 20.09 & 19.54 &   \\
H20-11721 & pff\_gc-090 & PFF090;GC0386;PFF-gc090;GC386;T17-1992 & 201.58555 & -43.055143 & 519 $\pm$ 56 & m & 19.44 & 18.74 & 1 \\
H20-11732 & GC0078 & AAT111406;AAT111406;T17-1292 & 201.23030 & -43.054323 & 552 $\pm$ 31 & o & 20.21 & 19.49 & 1 \\
H20-11733 & pff\_gc-022 & PFF022;GC0073;PFF-gc022;GC073;pff\_gc-022;0073;T17-1283 & 201.22633 & -43.054294 & 557 $\pm$ 60 & o & 19.79 & 19.35 & 1 \\
H20-11745 & C138 & GC0173;GC173;T17-1495 & 201.32053 & -43.052217 &   &    & 20.54 & 20.01 &   \\
H20-11747 & C160 & GC0267;GC0267;T17-1684 & 201.41694 & -43.051880 & 480 $\pm$ 256 & p & 19.75 & 19.43 &   \\
H20-11761 & HGHH-G66 & HGHH-G066;G066;GC0110;GC110;G066;GC0110;T17-1370 & 201.26320 & -43.050690 & 577 $\pm$ 5 & p & 18.77 & 18.09 &   \\
H20-11770 & GC603 & GC0603;T17-1997 & 201.58805 & -43.049822 & 506 $\pm$ 56 & p & 20.36 & 19.74 & 1 \\
H20-11771 & GC530 & GC0530;T17-1803 & 201.46901 & -43.050018 & 488 $\pm$ 50 & p & 21.15 & 20.37 &   \\
H20-11779 &           47 & WHH-9;WHH09;GC0130;GC130;WHH-9;GC0130;T17-1416 & 201.28550 & -43.049289 & 361 $\pm$ 12 & p & 18.98 & 18.26 &   \\
H20-11785 & HCH13 & GC0206;HCH13;T17-1574 & 201.36953 & -43.048587 & 613 $\pm$ 37 & m & 19.21 & 18.45 &   \\
H20-11790 & GC537 & GC0537;T17-1839 & 201.48394 & -43.048151 & 398 $\pm$ 30 & p & 21.31 & 20.38 & 1 \\
H20-11792 & GC0450 &  & 201.22921 & -43.048040 & 415 $\pm$ 92 & o & 20.30 & 19.90 & 1 \\
H20-11800 & C141 & GC0179;T17-1504 & 201.32560 & -43.047463 &   &    & 21.19 & 20.65 &   \\
H20-11804 & C150 & GC0235;GC235;GC0235;T17-1622 & 201.39094 & -43.047063 & 607 $\pm$ 31 & p & 22.16 & 20.19 &   \\
H20-11810 &           75 & WHH-5;GC0050;WHH-5;GC0050;0050;T17-1223 & 201.18578 & -43.046455 & 718 $\pm$ 16 & p & 19.08 & 18.42 & 1 \\
H20-11828 & GC585 & GC0585;T17-1466 & 201.30866 & -43.045179 & 510 $\pm$ 82 & p & 20.23 & 19.75 &   \\
H20-11853 & C134 & GC0152;GC152;T17-1459 & 201.30509 & -43.042024 &   &    & 20.71 & 20.21 &   \\
H20-11859 & HGHH-G331 & HGHH-G331;GC0184;HGHH-G331;GC0184;T17-1517 & 201.33121 & -43.041221 & 371 $\pm$ 14 & p & 18.92 & 18.53 &   \\
H20-11867 & GC0053 & AAT109788;GC053;AAT109788;GC0053;0053;T17-1229 & 201.19067 & -43.040134 & 503 $\pm$ 17 & p & 20.06 & 19.28 & 1 \\
H20-11879 & C137 & GC0166;GC0166;T17-1482 & 201.31694 & -43.038577 & 467 $\pm$ 34 & p & 19.26 & 18.66 &   \\
H20-11887 & GC420 & LDSS2-30676;GC0420;0420;T17-1299 & 201.23327 & -43.037725 & 735 $\pm$ 28 & p & 20.26 & 19.76 & 1 \\
H20-11903 & HCH02 & GC0171;HCH02;0171;T17-1492 & 201.31949 & -43.035752 & 483 $\pm$ 50 & m & 18.66 & 18.06 &   \\
H20-11907 &          122 & GC0031;AAT107145;GC0031;0031;T17-1165 & 201.12378 & -43.035130 & 595 $\pm$ 202 & p & 20.08 & 19.51 & 1 \\
H20-11910 & HGHH-G204 & HGHH-G204;GC0298;HGHH-G204;T17-1752 & 201.44579 & -43.034827 & 705 $\pm$ 36 & m & 18.22 & 17.72 &   \\
H20-11914 & GC0454 & GC0454;T17-1366 & 201.26177 & -43.034552 & 399 $\pm$ 24 & p & 19.84 & 19.11 &   \\
H20-11923 & HGHH-G256 & HGHH-G256;G256;GC0322;HGHH-G256;GC322;GC0322;T17-1807 & 201.47031 & -43.033344 & 478 $\pm$ 13 & p & 19.15 & 18.32 &   \\
H20-11928 & GC445 & GC0445;GC0445;T17-1205 & 201.16882 & -43.032416 & 325 $\pm$ 29 & p & 20.65 & 20.00 & 1 \\
H20-11944 & pff\_gc-015 & PFF015;GC0046;PFF-gc015;GC046;pff\_gc-015;GC0046;T17-1210 & 201.17162 & -43.029332 & 518 $\pm$ 18 & p & 19.12 & 18.62 & 1 \\
H20-11957 & GC531 & GC0531;T17-1823 & 201.47822 & -43.027890 & 341 $\pm$ 23 & p & 21.18 & 20.18 & 1 \\
H20-11962 & GC0568 & T17-1159 & 201.11747 & -43.026789 & 211 $\pm$ 16 & p & 20.43 & 19.70 &   \\
H20-11970 & GC0455 & GC0455;T17-1389 & 201.27098 & -43.025931 & 498 $\pm$ 27 & p & 20.59 & 19.90 &   \\
H20-11974 & C133 & GC0141;GC141;T17-1436 & 201.29610 & -43.025531 &   &    & 19.84 & 19.00 &   \\
H20-11985 & HGHH-11 & C11;C11;HGHH-11;C11;C11;HGHH92-C11;GC0077;HGHH-11;GC077;C11;GC0077;0077;T17-1287 & 201.22799 & -43.022687 & 791 $\pm$ 1 & p & 17.94 & 17.21 & 1 \\
H20-11987 & HGHH-42 & HGHH-42;C42;GC0066;HGHH-42;GC066;GC0066;T17-1260 & 201.21190 & -43.023016 & 550 $\pm$ 10 & p & 18.96 & 18.23 & 1 \\
H20-11988 & pff\_gc-088 & PFF088;GC0374;PFF-gc088;GC374;T17-1946 & 201.53689 & -43.022600 & 546 $\pm$ 50 & m & 18.91 & 18.42 & 1 \\
H20-11995 & HGHH-9 & HGHH-09;C9;GC0055;GC055;T17-1232 & 201.19459 & -43.021772 & 501 $\pm$ 21 & l & 18.90 & 18.40 & 1 \\
H20-12011 & HGHH-31 & C31;C31;HGHH-31;C31;GC0086;HGHH-31;GC086;C31;GC0086;T17-1313 & 201.23929 & -43.018916 & 685 $\pm$ 9 & p & 18.50 & 17.77 & 1 \\
H20-12044 & C135 & GC0156;GC0156;T17-1467 & 201.30869 & -43.014287 & 577 $\pm$ 55 & p & 18.96 & 18.51 &   \\
H20-12049 & MAGJM-01 & GC0263;MAGJM-01;T17-1678 & 201.41386 & -43.013542 & 603 $\pm$ 48 & m & 19.74 & 19.07 &   \\
H20-12053 & pff\_gc-094 & PFF094;GC0396;PFF-gc094;T17-2012 & 201.59856 & -43.012646 & 372 $\pm$ 144 & m & 19.94 & 19.41 & 1 \\
H20-12057 &          140 & GC449;GC0449;GC0449;T17-1277 & 201.22490 & -43.012107 & 362 $\pm$ 22 & p & 20.32 & 19.57 & 1 \\
H20-12059 & HGHH-G357 & HGHH-G357;G357;GC0300;GC300;G357;T17-1758 & 201.44908 & -43.012041 & 748 $\pm$ 33 & o & 19.69 & 19.17 &   \\
H20-12063 & GC594 & GC0594;T17-1829 & 201.47946 & -43.011574 & 630 $\pm$ 87 & p & 20.30 & 19.80 & 1 \\
H20-12070 & pff\_gc-085 & PFF085;pff\_gc-085;GC0367;PFF-gc085;GC367;pff\_gc-085;0367;T17-1926 & 201.52673 & -43.010570 & 557 $\pm$ 40 & o & 19.37 & 18.90 & 1 \\
H20-12081 &          182 & GC0313;AAT120355;GC313;AAT120355;T17-1785 & 201.45986 & -43.009059 & 729 $\pm$ 74 & o & 20.32 & 19.94 &   \\
H20-12119 & GC0355 & AAT122445;0355;T17-1896 & 201.51010 & -43.003235 & 342 $\pm$ 98 & m & 20.17 & 19.72 & 1 \\
H20-12124 & pff\_gc-030 & PFF030;GC0105;pff\_gc-030;0105;T17-1357 & 201.25716 & -43.002728 & 306 $\pm$ 48 & o & 19.97 & 19.20 &   \\
H20-12141 & HCH99-18 & HCH18;HCH99-18;GC0225;HCH18;0225;T17-1608 & 201.38167 & -43.000772 & 550 $\pm$ 45 & m & 17.45 & 16.97 &   \\
H20-12142 & HCH99-15 & HCH99-15;GC0213;0213;T17-1586 & 201.37467 & -43.001396 & 519 $\pm$ 1 & l & 18.29 & 17.73 &   \\
H20-12144 & GC0569 & T17-1164 & 201.12303 & -43.000961 & 586 $\pm$ 30 & p & 19.57 & 18.89 & 1 \\
H20-12161 & MAGJM-06 &          313;GC0254;MAGJM-06;T17-1658 & 201.40288 & -42.999756 & 487 $\pm$ 37 & m & 18.93 & 18.20 &   \\
H20-12162 & GC0447 &  & 201.21205 & -42.999608 & 607 $\pm$ 77 & o & 21.18 & 20.72 & 1 \\
H20-12164 & GC0479 &  & 201.49992 & -42.999434 & 525 $\pm$ 86 & o & 20.86 & 20.42 & 1 \\
H20-12166 & GC0469 &  & 201.38232 & -42.999336 & 377 $\pm$ 39 & o & 20.29 & 19.66 &   \\
H20-12188 & pff\_gc-020 & PFF020;GC0065;pff\_gc-020;0065;T17-1259 & 201.21030 & -42.996933 & 250 $\pm$ 48 & o & 19.45 & 18.94 &   \\
H20-12189 & pff\_gc-014 & PFF014;GC0045;PFF-gc014;GC045;T17-1209 & 201.17100 & -42.996765 & 718 $\pm$ 59 & m & 20.26 & 19.65 & 1 \\
H20-12190 & GC451 & GC0451;GC0451;T17-1295 & 201.23096 & -42.996797 & 656 $\pm$ 32 & p & 19.92 & 19.37 & 1 \\
H20-12192 & pff\_gc-071 & PFF071;GC0317;pff\_gc-071;T17-1795 & 201.46474 & -42.996333 & 398 $\pm$ 51 & o & 19.74 & 19.25 & 1 \\
H20-12197 & HCH99-1 & HCH01;HCH99-2;GC0168;HCH01;T17-1485 & 201.31758 & -42.995375 & 629 $\pm$ 78 & m & 19.24 & 18.65 &   \\
H20-12207 & MAGJM-11 & GC0237;MAGJM-11;T17-1626 & 201.39142 & -42.994249 & 508 $\pm$ 51 & m & 19.17 & 18.46 &   \\
H20-12216 & HCH99-16 & HCH16;HCH99-16;GC0217;HCH16;0217;T17-1594 & 201.37621 & -42.992968 & 518 $\pm$ 45 & m & 18.81 & 18.37 &   \\
H20-12229 &          115 & GC0316;AAT120515;AAT120515;0316;T17-1794 & 201.46374 & -42.991484 & 316 $\pm$ 39 & o & 19.88 & 19.30 & 1 \\
H20-12241 & HGHH-G369 & HGHH-G369;G369;G369;GC0087;HGHH-G369;GC087;G369;T17-1314 & 201.23962 & -42.989794 & 481 $\pm$ 22 & o & 18.72 & 18.20 & 1 \\
H20-12249 & HGHH-G268 & HGHH-G268;G268;GC0260;T17-1672 & 201.41087 & -42.988730 & 436 $\pm$ 43 & l & 18.96 & 18.35 &   \\
H20-12250 & GC0456 & GC0456;T17-1402 & 201.27801 & -42.988084 & 443 $\pm$ 19 & p & 18.65 & 18.22 &   \\
H20-12251 & GC0373 & AAT123453;GC0373;0373;T17-1944 & 201.53488 & -42.988540 & 586 $\pm$ 46 & p & 20.08 & 19.52 & 1 \\
H20-12255 & HGHH-G370 & HGHH-G370;G370;GC0277;HGHH-G370;G370;0277;T17-1708 & 201.42605 & -42.988014 & 471 $\pm$ 24 & o & 18.40 & 17.82 &   \\
H20-12258 & C103 & GC0331;C103;T17-1831 & 201.47922 & -42.987156 & 548 $\pm$ 17 & o & 19.06 & 18.32 & 1 \\
H20-12261 & C102 & GC0318;T17-1800 & 201.46710 & -42.986906 &   &    & 21.44 & 20.72 &   \\
H20-12268 & C22 & C22;HGHH-22;C22;HGHH92-C22;GC0326;HGHH-22;C22;GC0326;T17-1814 & 201.47318 & -42.985402 & 577 $\pm$ 89 & p & 18.16 & 17.58 & 1 \\
H20-12271 & GC0134 & K-029;K-029;T17-1423 & 201.28831 & -42.983084 & 630 $\pm$ 33 & o & 17.76 & 17.24 &   \\
H20-12274 & pff\_gc-057 & PFF057;GC0234;GC0234;0234;T17-1621 & 201.38822 & -42.984189 & 518 $\pm$ 10 & p & 20.44 & 19.67 &   \\
H20-12275 & pff\_gc-060 & PFF060;pff\_gc-060;GC0278;pff\_gc-060;0278;T17-1711 & 201.42680 & -42.984012 & 848 $\pm$ 22 & o & 18.83 & 18.21 &   \\
H20-12277 & HGHH-G342 & HGHH-G342;G342;GC0124;HGHH-G342;G342;T17-1397 & 201.27425 & -42.983471 & 481 $\pm$ 27 & o & 18.22 & 17.58 &   \\
H20-12280 & HGHH-35 & C35;GC0286;GC286;C35;T17-1724 & 201.43422 & -42.983142 & 550 $\pm$ 34 & o & 18.62 & 18.00 &   \\
H20-12287 & GC0574 & T17-1221 & 201.18442 & -42.981737 & 512 $\pm$ 30 & p & 20.93 & 20.26 & 1 \\
H20-12290 & GC452 & GC0452;GC0452;T17-1318 & 201.24070 & -42.981000 & 643 $\pm$ 39 & p & 21.27 & 20.71 & 1 \\
H20-12298 & HGHH-G219 & HGHH-G219;GC0176;HGHH-G219;T17-1498 & 201.32210 & -42.979603 & 534 $\pm$ 28 & m & 18.92 & 18.19 &   \\
H20-12302 & pff\_gc-073 & PFF073;pff\_gc-073;GC0321;PFF-gc073;pff\_gc-073;GC0321;0321;T17-1806 & 201.46991 & -42.978214 & 348 $\pm$ 22 & p & 20.01 & 19.34 & 1 \\
H20-12306 & GC520 & GC0520;T17-1568 & 201.36331 & -42.977193 & 572 $\pm$ 48 & p & 20.78 & 20.12 &   \\
H20-12307 & pff\_gc-062 & PFF062;GC0281;pff\_gc-062;GC0281;T17-1718 & 201.43011 & -42.977014 & 691 $\pm$ 19 & p & 19.50 & 18.77 &   \\
H20-12309 & GC0467 & T17-1602 & 201.37903 & -42.976903 & 209 $\pm$ 33 & o & 19.01 & 18.80 &   \\
H20-12314 &          164 & GC0550;T17-2033 & 201.62127 & -42.975316 & 818 $\pm$ 45 & p & 20.46 & 19.88 & 1 \\
H20-12316 & pff\_gc-072 & PFF072;GC0319;pff\_gc-072;GC0319;T17-1801 & 201.46724 & -42.975001 & 475 $\pm$ 18 & p & 19.63 & 19.06 & 1 \\
H20-12317 & HGHH-G277 & HGHH-G277;G277;GC0057;HGHH-G277;GC057;G277;T17-1235 & 201.19735 & -42.974939 & 714 $\pm$ 31 & o & 19.10 & 18.55 & 1 \\
H20-12319 & C175 & GC0348;T17-1880 & 201.50395 & -42.974684 &   &    & 22.37 & 21.72 &   \\
H20-12321 & GC463 & GC0463;GC0463;T17-1569 & 201.36370 & -42.974658 & 237 $\pm$ 30 & p & 19.76 & 19.08 &   \\
H20-12323 & GC0185 & AAT115561;GC185;T17-1521 & 201.33259 & -42.974198 & 514 $\pm$ 46 & m & 20.64 & 19.97 &   \\
H20-12327 & GC0474 &  & 201.43646 & -42.973574 & 376 $\pm$ 75 & o & 21.02 & 20.32 &   \\
H20-12328 & GC0527 & T17-1679 & 201.41423 & -42.973357 & 301 $\pm$ 19 & p & 20.15 & 19.67 &   \\
H20-12334 & GC0196 & AAT116385;GC196;T17-1555 & 201.35579 & -42.972592 & 550 $\pm$ 40 & m & 20.41 & 19.79 &   \\
H20-12337 & GC453 & GC0453;GC0453;T17-1327 & 201.24416 & -42.971258 & 620 $\pm$ 9 & p & 19.07 & 18.36 & 1 \\
H20-12338 & pff\_gc-017 & PFF017;GC0049;GC049;pff\_gc-017;T17-1218 & 201.18175 & -42.971200 & 442 $\pm$ 53 & o & 19.49 & 18.98 & 1 \\
H20-12340 & GC578 & GC0578;T17-1294 & 201.23071 & -42.970827 & 385 $\pm$ 27 & p & 21.08 & 20.35 & 1 \\
H20-12341 & pff\_gc-083 & PFF083;pff\_gc-083;PFF083;GC0353;PFF-gc083;GC0353;0353;T17-1891 & 201.50760 & -42.970804 & 458 $\pm$ 31 & p & 19.90 & 19.26 & 1 \\
H20-12345 & GC0273 & AAT118874;AAT118874;GC0273;0273;T17-1697 & 201.42233 & -42.969123 & 774 $\pm$ 35 & p & 20.13 & 19.48 &   \\
H20-12347 & GC0147 & AAT114302;GC147;0147;T17-1448 & 201.30140 & -42.968776 & 754 $\pm$ 143 & m & 20.48 & 19.87 &   \\
H20-12350 & HGHH-G35 & HGHH-G035;G035;GC0121;GC121;G035;GC0121;0121;T17-1391 & 201.27199 & -42.968252 & 787 $\pm$ 19 & p & 19.68 & 19.02 & 1 \\
H20-12351 & GC581 & GC0581;T17-1328 & 201.24436 & -42.968191 & 524 $\pm$ 74 & p & 20.26 & 19.88 & 1 \\
H20-12357 & pff\_gc-070 & PFF070;GC0314;pff\_gc-070;GC0314;0314;T17-1786 & 201.46001 & -42.967283 & 585 $\pm$ 22 & p & 19.38 & 18.89 & 1 \\
H20-12359 & GC0570 & T17-1185 & 201.14640 & -42.966532 & 297 $\pm$ 21 & p & 19.95 & 19.41 & 1 \\
H20-12360 & GC448 & GC0448;GC0448;T17-1276 & 201.22352 & -42.966389 & 633 $\pm$ 23 & p & 20.72 & 20.05 & 1 \\
H20-12364 & GC0028 & AAT106880;GC0028;0028;T17-1160 & 201.11845 & -42.964690 & 558 $\pm$ 97 & p & 20.08 & 19.60 & 1 \\
H20-12368 &           91 & WHH-6;GC0058;WHH-06;GC058;0058;T17-1234 & 201.19737 & -42.964193 & 666 $\pm$ 56 & m & 19.82 & 19.13 & 1 \\
H20-12371 & GC0476 &  & 201.44615 & -42.963752 & 482 $\pm$ 45 & o & 19.65 & 19.21 & 1 \\
H20-12374 & pff\_gc-019 & PFF019;GC0062;GC062;pff\_gc-019;GC0062;T17-1252 & 201.20400 & -42.963438 & 611 $\pm$ 17 & p & 18.97 & 18.47 & 1 \\
H20-12378 &           40 & WHH-17;GC0208;WHH-17;GC208;WHH-17;T17-1580 & 201.37190 & -42.963073 & 658 $\pm$ 32 & o & 18.54 & 18.01 &   \\
H20-12380 & GC0161 & AAT114769;GC161;AAT114769;0161;T17-1475 & 201.31295 & -42.962662 & 541 $\pm$ 61 & o & 20.18 & 19.72 &   \\
H20-12385 & pff\_gc-032 & PFF032;GC0111;PFF-gc032;GC111;GC0111;T17-1371 & 201.26347 & -42.961243 & 648 $\pm$ 29 & p & 19.75 & 19.18 & 1 \\
H20-12391 & HGHH-G170 & HGHH-G170;G170;G170;GC0370;HGHH-G170;G170;GC0370;T17-1933 & 201.52886 & -42.959714 & 652 $\pm$ 8 & p & 19.30 & 18.61 & 1 \\
H20-12392 & GC496 & GC0496;T17-1336 & 201.24917 & -42.959212 & 581 $\pm$ 18 & p & 20.10 & 19.61 & 1 \\
H20-12393 & GC0477 &  & 201.44943 & -42.958852 & 335 $\pm$ 66 & o & 21.80 & 21.07 & 1 \\
H20-12398 & GC0441 & 0441;T17-1820 & 201.47705 & -42.957651 & 603 $\pm$ 10 & p & 19.70 & 19.01 & 1 \\
H20-12399 & GC0488 & T17-1154 & 201.11344 & -42.957100 & 559 $\pm$ 35 & p & 21.53 & 20.88 & 1 \\
H20-12400 & HGHH-G81 & HGHH-G081;G081;GC0145;GC145;G081;GC0145;T17-1445 & 201.30043 & -42.956994 & 490 $\pm$ 10 & p & 18.61 & 18.02 & 1 \\
H20-12402 & GC471 & GC0471;GC0471;T17-1706 & 201.42548 & -42.956642 & 275 $\pm$ 24 & p & 19.56 & 19.23 & 1 \\
H20-12404 &           33 & WHH-23;GC0289;GC289;WHH-23;GC0289;0289;T17-1734 & 201.44131 & -42.955584 & 286 $\pm$ 63 & l & 18.25 & 17.82 & 1 \\
H20-12406 & GC435 & GC0435;0435;T17-1671 & 201.41057 & -42.955528 & 706 $\pm$ 63 & p & 19.90 & 19.19 & 1 \\
H20-12407 & pff\_gc-092 & PFF092;N26;GC0390;PFF-gc092;GC0390;T17-1999 & 201.58876 & -42.955285 & 453 $\pm$ 23 & p & 19.99 & 19.34 & 1 \\
H20-12409 & GC430 & GC0430;T17-1550 & 201.35161 & -42.954660 & 503 $\pm$ 75 & p & 19.53 & 18.82 &   \\
H20-12422 & pff\_gc-095 & PFF095;GC0400;PFF-gc095;GC0400;T17-2023 & 201.60624 & -42.951689 & 406 $\pm$ 18 & p & 19.65 & 18.98 & 1 \\
H20-12423 & C176 & GC0356;GC0356;T17-1898 & 201.51168 & -42.951348 & 326 $\pm$ 93 & p & 21.42 & 21.09 & 1 \\
H20-12426 & HGHH-G284 & HGHH-G284;G284;G284;GC0295;HGHH-G284;GC295;G284;GC0295;0295;T17-1747 & 201.44412 & -42.950784 & 471 $\pm$ 10 & p & 19.98 & 19.30 & 1 \\
H20-12427 & HGHH-45 & C45;GC0239;HGHH-45;GC239;C45;0239;T17-1630 & 201.39273 & -42.949694 & 591 $\pm$ 39 & o & 18.82 & 18.37 & 1 \\
H20-12428 &           88 & WHH-10;GC0149;GC149;GC0149;0149;T17-1453 & 201.30352 & -42.949940 & 664 $\pm$ 141 & p & 19.51 & 19.02 & 1 \\
H20-12429 & C25 & C25;HGHH-25;C25;C25;GC0357;HGHH-25;GC357;GC0357;T17-1899 & 201.51185 & -42.949146 & 702 $\pm$ 6 & p & 18.57 & 17.80 & 1 \\
H20-12431 &           96 & WHH-24;GC0291;GC291;WHH-24;GC0291;0291;T17-1738 & 201.44171 & -42.948037 & 606 $\pm$ 30 & p & 19.59 & 19.11 & 1 \\
H20-12432 & pff\_gc-028 & PFF028;GC001;GC0001;T17-1347 & 201.25480 & -42.947642 & 516 $\pm$ 10 & p & 18.80 & 18.19 & 1 \\
H20-12433 & GC583 & GC0583;T17-1362 & 201.25916 & -42.947628 & 602 $\pm$ 84 & p & 20.65 & 20.06 & 1 \\
H20-12437 &           28 & WHH-18;GC0215;WHH-18;GC215;WHH-18;T17-1588 & 201.37534 & -42.946344 & 761 $\pm$ 13 & o & 18.44 & 17.79 & 1 \\
H20-12438 & C178 & GC0360;T17-1908 & 201.51610 & -42.945923 &   &    & 21.77 & 21.27 &   \\
H20-12439 & pff\_gc-058 & PFF058;pff\_gc-058;GC0245;PFF-gc058;GC245;pff\_gc-058;GC0245;T17-1640 & 201.39637 & -42.945864 & 333 $\pm$ 14 & p & 18.61 & 18.14 & 1 \\
H20-12440 & C106 & GC0366;GC366;T17-1924 & 201.52583 & -42.945555 &   &    & 21.47 & 20.75 &   \\
H20-12445 & C179 & GC0377;GC377;T17-1953 & 201.54119 & -42.943320 &   &    & 21.18 & 20.86 &   \\
H20-12451 &          138 & WHH-14;GC0197;WHH-14;GC197;WHH-14;GC0197;0197;T17-1556 & 201.35625 & -42.941990 & 597 $\pm$ 34 & p & 20.03 & 19.54 & 1 \\
H20-12454 & GC434 & GC0434;T17-1664 & 201.40775 & -42.941098 & 480 $\pm$ 16 & p & 18.98 & 18.31 & 1 \\
H20-12455 & HGHH-G176 & HGHH-G176;G176;GC0109;HGHH-G176;GC109;G176;GC0109;T17-1369 & 201.26302 & -42.940278 & 523 $\pm$ 8 & p & 19.01 & 18.32 & 1 \\
H20-12456 & pff\_gc-056 & PFF056;pff\_gc-056;GC0231;GC231;pff\_gc-056;T17-1617 & 201.38670 & -42.940074 & 254 $\pm$ 33 & o & 18.57 & 18.09 & 1 \\
H20-12460 &          160 & AAT120976;GC0328;AAT120976;GC328;AAT120976;T17-1816 & 201.47621 & -42.939005 & 670 $\pm$ 51 & o & 20.33 & 19.75 & 1 \\
H20-12463 & VHH81-03 & C3;C3;C3;VHH81-C3;GC0091;VHH81-03;GC091;C3;GC0091;T17-1322 & 201.24254 & -42.936099 & 561 $\pm$ 1 & p & 17.71 & 17.03 & 1 \\
H20-12465 & GC459 & GC0459;T17-1502 & 201.32367 & -42.937162 & 458 $\pm$ 72 & o & 21.68 & 21.04 & 1 \\
H20-12474 & C17 & C17;HGHH-17;C17;C17;HGHH92-C17;GC0265;HGHH-17;GC265;C17;GC0265;0265;T17-1682 & 201.41555 & -42.933070 & 780 $\pm$ 1 & p & 17.61 & 17.06 & 1 \\
H20-12475 & C101 &          170;GC0268;GC268;GC0268;T17-1687 & 201.41903 & -42.933607 & 631 $\pm$ 91 & p & 20.57 & 19.91 & 1 \\
H20-12478 & GC507 & GC0507;T17-1456 & 201.30434 & -42.932285 & 461 $\pm$ 27 & p & 19.98 & 19.52 & 1 \\
H20-12481 &          152 & GC0301;AAT119894;T17-1759 & 201.44965 & -42.931149 & 448 $\pm$ 90 & m & 20.25 & 19.53 & 1 \\
H20-12483 & GC458 & GC0458;GC0458;T17-1413 & 201.28214 & -42.930413 & 533 $\pm$ 32 & p & 20.94 & 20.77 & 1 \\
H20-12485 &          220 & C119;GC0089;GC089;T17-1317 & 201.24039 & -42.930081 &   &    & 20.47 & 20.49 &   \\
H20-12487 & GC468 & GC0468;T17-1606 & 201.38030 & -42.929911 & 372 $\pm$ 68 & o & 21.55 & 20.86 & 1 \\
H20-12488 & HGHH-G293 & G293;HGHH-G293;G293;G293;GC0361;HGHH-G293;GC361;GC0361;T17-1910 & 201.51748 & -42.929053 & 583 $\pm$ 10 & p & 19.10 & 18.60 & 1 \\
H20-12491 &          198 & C169;GC0315;GC315;0315;T17-1793 & 201.46261 & -42.926719 &   &    & 20.46 & 20.13 &   \\
H20-12492 &          221 & C171;GC0336;T17-1856 & 201.49079 & -42.926652 &   &    & 21.03 & 20.44 &   \\
H20-12495 & C104 & C104/AAT121826;GC0342;AAT121826;GC342;GC0342;T17-1867 & 201.49784 & -42.925183 & 448 $\pm$ 97 & p & 19.78 & 19.25 & 1 \\
H20-12496 & GC464 & GC0464;GC0464;T17-1570 & 201.36435 & -42.925018 & 461 $\pm$ 35 & p & 21.02 & 20.36 & 1 \\
H20-12498 & GC593 & GC0593;T17-1799 & 201.46699 & -42.924484 & 223 $\pm$ 26 & p & 20.20 & 19.60 &   \\
H20-12502 & f1.GC-20 & f1.GC20;GC0542;T17-1919 & 201.52243 & -42.922865 & 364 $\pm$ 47 & p & 21.57 & 20.88 & 1 \\
H20-12507 & pff\_gc-040 & PFF040;GC0135;GC135;GC0135;T17-1426 & 201.28971 & -42.921783 & 448 $\pm$ 23 & p & 19.05 & 18.58 & 1 \\
H20-12509 & C174 & GC0345;T17-1871 & 201.49852 & -42.920997 &   &    & 21.80 & 21.06 &   \\
H20-12510 &          142 & GC0226;AAT117322;GC226;AAT117322;0226;T17-1610 & 201.38221 & -42.920995 & 636 $\pm$ 133 & m & 20.01 & 19.50 & 1 \\
H20-12512 & HGHH-G221 & G221;HGHH-G221;G221;G221;GC0351;GC0351;T17-1884 & 201.50460 & -42.920374 & 383 $\pm$ 12 & p & 19.39 & 18.74 & 1 \\
H20-12515 & GC528 & GC0528;T17-1762 & 201.45137 & -42.918538 & 489 $\pm$ 19 & p & 20.36 & 19.67 & 1 \\
H20-12520 & f1.GC-22 & R122;GC0382;GC0382;0382;T17-1974 & 201.56617 & -42.916896 & 587 $\pm$ 1 & p & 18.00 & 17.55 & 1 \\
H20-12521 & C173 & GC0344;T17-1869 & 201.49824 & -42.917052 &   &    & 21.57 & 20.86 &   \\
H20-12527 & GC470 & GC0470 & 201.38797 & -42.915893 & 624 $\pm$ 74 & o & 20.90 & 20.39 & 1 \\
H20-12529 & GC589 & GC0589;T17-1667 & 201.40951 & -42.914907 & 686 $\pm$ 98 & p & 20.44 & 19.71 & 1 \\
H20-12531 & HGHH-20 & C20;C20;GC0306;HGHH-20;GC0306;0306;T17-1773 & 201.45706 & -42.913666 & 738 $\pm$ 6 & p & 17.93 & 17.37 & 1 \\
H20-12532 & pff\_gc-021 & PFF021;PFF021;GC0072;GC072;GC0072;T17-1280 & 201.22570 & -42.913991 & 564 $\pm$ 33 & p & 19.16 & 18.69 & 1 \\
H20-12538 & pff\_gc-053 & PFF053;GC0211;GC211;pff\_gc-053;T17-1584 & 201.37345 & -42.912328 & 390 $\pm$ 18 & o & 19.35 & 18.66 & 1 \\
H20-12539 & pff\_gc-029 & PFF029;PFF029;GC0103;GC103;GC0103;0103;T17-1355 & 201.25665 & -42.911317 & 603 $\pm$ 32 & p & 19.00 & 18.96 & 1 \\
H20-12547 & C117 & GC0082;GC082;GC0082;0082;T17-1300 & 201.23360 & -42.908194 & 529 $\pm$ 26 & p & 19.94 & 19.20 & 1 \\
H20-12550 & R118 & GC0392;GC392;T17-2003 & 201.59169 & -42.907318 & 440 $\pm$ 73 & l & 19.79 & 19.34 & 1 \\
H20-12553 & GC437 & GC0437;0437;T17-1729 & 201.43849 & -42.906602 & 490 $\pm$ 113 & p & 20.62 & 19.91 & 1 \\
H20-12564 & GC0096 & AAT112158;GC096;0096;T17-1339 & 201.25062 & -42.902458 & 699 $\pm$ 43 & m & 20.54 & 19.89 & 1 \\
H20-12565 &          175 & GC0187;AAT115605;GC187;GC0187;0187;T17-1527 & 201.33518 & -42.902328 & 855 $\pm$ 73 & p & 20.46 & 19.99 & 1 \\
H20-12567 & HHH86-38 & C38;C38;HHH86-C38=R123;GC0397;GC0397;0397;T17-2013 & 201.59909 & -42.900267 & 405 $\pm$ 1 & p & 18.48 & 17.88 & 1 \\
H20-12569 &          155 & GC588;GC0588;T17-1590 & 201.37565 & -42.900241 & 1051 $\pm$ 52 & p & 20.25 & 19.77 & 1 \\
H20-12577 & GC0296 & AAT119697;GC296;GC0296;T17-1748 & 201.44448 & -42.896768 & 633 $\pm$ 108 & p & 20.15 & 19.46 & 1 \\
H20-12579 & R117 & GC0391;R117;GC391;GC0391;T17-2002 & 201.59164 & -42.895943 & 459 $\pm$ 23 & p & 19.64 & 19.19 & 1 \\
H20-12580 & C37 & C37;HGHH-37;C37;C37;C37;HGHH92-C37=R116;GC0378;HGHH-37;GC378;GC0378;0378;T17-1957 & 201.54408 & -42.895154 & 612 $\pm$ 1 & p & 18.52 & 17.88 & 1 \\
H20-12582 & GC534 & GC0534;T17-1832 & 201.48066 & -42.894496 & 347 $\pm$ 41 & p & 20.89 & 20.42 & 1 \\
H20-12583 &          139 & GC0252;AAT117899;GC252;0252;T17-1652 & 201.40030 & -42.894495 & 609 $\pm$ 116 & m & 20.22 & 19.56 & 1 \\
H20-12587 & GC0138 & K-034;GC138;GC0138;T17-1430 & 201.29279 & -42.892480 & 416 $\pm$ 8 & p & 17.82 & 17.16 & 1 \\
H20-12595 &          172 & GC0209;AAT116969;GC209;0209;T17-1581 & 201.37255 & -42.890417 & 446 $\pm$ 61 & m & 20.43 & 19.92 & 1 \\
H20-12600 & pff\_gc-079 & PFF079;PFF079;GC0341;PFF-gc079;GC341;GC0341;0341;T17-1864 & 201.49544 & -42.888540 & 410 $\pm$ 20 & p & 19.61 & 19.05 & 1 \\
H20-12601 & f1.GC-14 & f1.GC14;GC442;GC0442;T17-1948 & 201.53907 & -42.888176 & 632 $\pm$ 52 & p & 20.01 & 19.49 & 1 \\
H20-12604 &          149 & GC521;GC0521;T17-1577 & 201.37005 & -42.887733 & 176 $\pm$ 24 & p & 20.38 & 19.71 &   \\
H20-12611 & pff\_gc-016 & PFF016;PFF016;GC0048;PFF-gc016;GC048;GC0048;0048;T17-1217 & 201.18162 & -42.885316 & 509 $\pm$ 15 & p & 19.93 & 19.25 & 1 \\
H20-12619 &           63 & WHH-12;GC0180;GC180;GC0180;T17-1506 & 201.32617 & -42.884639 & 384 $\pm$ 16 & p & 19.07 & 18.47 & 1 \\
H20-12620 & C172 & GC0337;T17-1858 & 201.49145 & -42.884518 &   &    & 21.24 & 20.82 &   \\
H20-12622 & VHH81-05 & VHH81-C5;GC0167;VHH81-05;T17-1483 & 201.31718 & -42.882779 & 563 $\pm$ 41 & m & 17.50 & 17.02 & 1 \\
H20-12623 & GC0246 & K-144;GC246;GC0246;0246;T17-1641 & 201.39651 & -42.883568 & 593 $\pm$ 43 & p & 20.44 & 19.70 & 1 \\
H20-12626 &          218 & GC532;GC0532;T17-1824 & 201.47830 & -42.882503 & 399 $\pm$ 32 & p & 21.16 & 20.44 & 1 \\
H20-12628 & GC510 & GC0510;T17-1503 & 201.32371 & -42.882326 & 670 $\pm$ 45 & p & 20.90 & 20.37 & 1 \\
H20-12636 & GC0518 & T17-1554 & 201.35574 & -42.824327 & 589 $\pm$ 63 & p & 21.22 & 20.73 & 1 \\
H20-12642 & GC0591 & T17-1781 & 201.45865 & -42.832779 & 702 $\pm$ 42 & p & 19.97 & 19.62 & 1 \\
H20-12649 &          119 & C115;GC0061;GC061;GC0061;T17-1248 & 201.20298 & -42.876508 & 509 $\pm$ 59 & p & 19.91 & 19.42 & 1 \\
H20-12652 & GC590 & GC0590;T17-1751 & 201.44572 & -42.876090 & 355 $\pm$ 66 & p & 19.86 & 19.24 & 1 \\
H20-12655 & GC0524 & T17-1625 & 201.39146 & -42.860916 & 527 $\pm$ 61 & p & 20.97 & 20.50 & 1 \\
H20-12661 & GC0440 & T17-1790 & 201.46085 & -42.861128 & 637 $\pm$ 32 & p & 19.16 & 18.73 & 1 \\
H20-12669 & HGHH-47 & C47;C47;GC0310;0310;T17-1780 & 201.45813 & -42.869214 & 589 $\pm$ 22 & l & 18.67 & 18.13 & 1 \\
H20-12676 & pff\_gc-050 & GC0172;GC0172;T17-1493 & 201.31969 & -42.838393 & 711 $\pm$ 30 & p & 20.39 & 19.80 & 1 \\
H20-12677 & pff\_gc-045 & PFF045;GC0153;GC153;GC0153;0153;T17-1460 & 201.30548 & -42.870060 & 474 $\pm$ 23 & p & 19.70 & 18.99 & 1 \\
H20-12680 &          103 & GC0431;0431;T17-1575 & 201.36971 & -42.836726 & 646 $\pm$ 24 & p & 19.61 & 19.16 & 1 \\
H20-12683 & HGHH-36 & C36;C36;C36;HGHH92-C36=R113;GC0372;HGHH-36;GC0372;0372;T17-1940 & 201.53220 & -42.866694 & 702 $\pm$ 1 & p & 18.36 & 17.83 & 1 \\
H20-12684 & R124 & GC0401;R124;T17-2031 & 201.62031 & -42.876719 & 599 $\pm$ 103 & m & 19.39 & 18.90 & 1 \\
H20-12689 &           54 & WHH-20;GC0240;WHH-20;GC0240;T17-1632 & 201.39321 & -42.851626 & 270 $\pm$ 27 & p & 19.02 & 18.43 & 1 \\
H20-12692 & HGHH-48 & C48;C48;GC0308;HGHH-48;GC0308;0308;T17-1777 & 201.45763 & -42.837519 & 557 $\pm$ 17 & p & 18.65 & 18.17 & 1 \\
H20-12693 &           53 & WHH-26;GC0334;GC0334;T17-1846 & 201.48590 & -42.862932 & 403 $\pm$ 16 & p & 19.14 & 18.48 & 1 \\
H20-12696 &           10 & WHH-19;GC0222;AAT117062;T17-1603 & 201.37934 & -42.837435 & 412 $\pm$ 71 & m & 17.23 & 16.69 & 1 \\
H20-12698 & GC0438 & 0438;T17-1735 & 201.44132 & -42.861436 & 837 $\pm$ 59 & p & 20.03 & 19.31 & 1 \\
H20-12702 & C120 & GC0090;GC090;T17-1320 & 201.24148 & -42.868045 &   &    & 21.93 & 21.29 &   \\
H20-12704 & pff\_gc-064 & PFF064;pff\_gc-064;GC0285;PFF-gc064;GC0285;0285;T17-1722 & 201.43292 & -42.845138 & 579 $\pm$ 20 & p & 19.77 & 19.10 & 1 \\
H20-12707 & pff\_gc-074 & PFF074;GC0324;PFF-gc074;GC0324;0324;T17-1811 & 201.47241 & -42.853369 & 470 $\pm$ 24 & p & 20.03 & 19.46 & 1 \\
H20-12708 & C32 & C32;HHH86-32;C32;C32;C32;GC0113;HHH86-32;GC113;GC0113;T17-1375 & 201.26402 & -42.846102 & 718 $\pm$ 10 & p & 18.50 & 17.77 & 1 \\
H20-12709 & pff\_gc-047 & PFF047;GC0160;GC160;GC0160;T17-1476 & 201.31302 & -42.841715 & 716 $\pm$ 55 & p & 19.84 & 19.32 & 1 \\
H20-12710 & C129 & GC0104;GC104;T17-1356 & 201.25678 & -42.847558 &   &    & 21.28 & 20.65 &   \\
H20-12724 & C130 & GC0107;GC107;GC0107;0107;T17-1360 & 201.25776 & -42.874367 & 635 $\pm$ 73 & p & 20.24 & 19.75 & 1 \\
H20-12725 &          121 & WHH-15;GC0203;WHH-15;GC203;GC0203;0203;T17-1566 & 201.36161 & -42.877727 & 508 $\pm$ 40 & p & 19.73 & 19.28 & 1 \\
H20-12727 & C131 & GC0115;GC115;GC0115;0115;T17-1378 & 201.26530 & -42.856010 & 425 $\pm$ 34 & p & 20.57 & 20.10 & 1 \\
H20-12730 & HHH86-33 & C33;GC0169;HHH86-33;GC0169;T17-1486 & 201.31777 & -42.848099 & 566 $\pm$ 13 & p & 18.48 & 17.96 & 1 \\
H20-58427 & GC0573 & T17-1207 & 201.17005 & -42.683759 & 517 $\pm$ 25 & p & 19.22 & 18.36 & 1 \\
H20-58446 & f1.GC-9 & GC0545;T17-2000 & 201.58903 & -42.833105 & 439 $\pm$ 28 & p & 21.07 & 20.63 & 1 \\
H20-58454 & C51 & GC0548;T17-2018 & 201.60077 & -42.783498 & 400 $\pm$ 12 & p & 18.73 & 18.20 & 1 \\
H20-58457 & pff\_gc-061 & PFF061;GC0280;PFF-gc061;T17-1713 & 201.42767 & -42.752975 & 508 $\pm$ 71 & m & 20.61 & 20.00 & 1 \\
H20-58469 & pff\_gc-069 & PFF069;GC0309;PFF-gc069;T17-1779 & 201.45809 & -42.668915 & 510 $\pm$ 71 & m & 20.27 & 19.58 & 1 \\
H20-58472 & pff\_gc-087 & PFF087;GC0369;PFF-gc087;T17-1932 & 201.52869 & -42.554765 & 856 $\pm$ 50 & m & 19.36 & 18.84 & 1 \\
H20-58473 & pff\_gc-099 & PFF099;GC0412;PFF-gc099;T17-2121 & 201.74933 & -42.544544 & 538 $\pm$ 80 & m & 20.18 & 19.70 & 1 \\
H20-58521 & GC0497 & T17-1345 & 201.25374 & -43.352118 & 478 $\pm$ 21 & p & 21.49 & 20.51 & 1 \\
H20-58524 & GC0329 & AAT328533;GC0329;T17-1819 & 201.47657 & -43.311159 & 673 $\pm$ 1 & p & 20.74 & 19.88 & 1 \\
H20-58789 & GC586 & GC0586;T17-1488 & 201.31893 & -43.103345 & 679 $\pm$ 45 & p & 21.10 & 20.27 &   \\
H20-58790 & GC0164 & AAT114913;GC164;AAT114913;GC0164;0164;T17-1480 & 201.31632 & -43.100923 & 570 $\pm$ 32 & p & 20.87 & 20.14 &   \\
H20-58795 & GC0503 & T17-1408 & 201.28075 & -43.056646 & 670 $\pm$ 41 & p & 20.52 & 19.95 &   \\
H20-58799 & C143 & GC0193;C143;T17-1544 & 201.34673 & -43.053567 & 328 $\pm$ 81 & o & 21.58 & 21.16 &   \\
H20-58800 & pff\_gc-041 & PFF041;pff\_gc-041;PFF041;GC0143;GC143;pff\_gc-041;GC0143;0143;T17-1441 & 201.29649 & -43.052653 & 426 $\pm$ 21 & p & 19.87 & 19.24 &   \\
H20-58806 & VHH81-06 & HGHH-6;HGHH-06;         308;C6;C6;HGHH92-C6;GC0191;HGHH-06;T17-1536 & 201.34245 & -43.045988 & 790 $\pm$ 44 & m & 17.60 & 16.92 &   \\
H20-58807 & C139 & GC0175;GC0175;0175;T17-1497 & 201.32112 & -43.045736 & 655 $\pm$ 16 & p & 19.77 & 18.95 &   \\
H20-58819 & GC500 & GC0500;T17-1377 & 201.26505 & -43.027934 & 386 $\pm$ 52 & p & 21.25 & 20.69 &   \\
H20-58820 & C142 & GC0182;GC0182;T17-1511 & 201.32714 & -43.021106 & 548 $\pm$ 19 & p & 18.51 & 17.52 &   \\
H20-58832 & GC473 & GC0473;T17-1716 & 201.42922 & -43.002021 & 318 $\pm$ 71 & o & 21.49 & 20.91 &   \\
H20-58841 & C23 & C23;HGHH-23;C23;HGHH92-C23;GC0330;HGHH-23;C23;GC0330;T17-1821 & 201.47742 & -42.990348 & 673 $\pm$ 1 & p & 17.73 & 16.96 & 1 \\
H20-58853 & HGHH-G169 & HGHH-G169;G169;GC0210;GC210;G169;0210;T17-1582 & 201.37262 & -42.969367 & 660 $\pm$ 34 & o & 19.96 & 19.10 &   \\
H20-58854 & HGHH-G292 & HGHH-G292;G292;GC0224;T17-1607 & 201.38118 & -42.968923 & 655 $\pm$ 43 & l & 20.53 & 19.66 &   \\
H20-58859 &            7 & WHH-7;GC0120;GC120;WHH-7;GC0120;T17-1388 & 201.27093 & -42.954215 & 677 $\pm$ 7 & p & 17.86 & 17.14 & 1 \\
H20-58867 & C7 & C7;HGHH-07;C7;C7;C7;HGHH92-C7;GC0365;HGHH-07;GC365;C7;GC0365;0365;T17-1920 & 201.52254 & -42.942304 & 594 $\pm$ 1 & p & 17.47 & 16.86 & 1 \\
H20-58877 & HHH86-30 & C30;C30;C30;GC0074;HHH86-30;GC074;GC0074;T17-1284 & 201.22648 & -42.890175 & 745 $\pm$ 7 & p & 17.68 & 16.98 & 1 \\
\hline
\end{tabular}
\caption{This is where the caption goes.}
\label{table:label_here}
\end{table*}

